InfoMerge: Information-aware Token Compression for Efficient Video Large Language Models

Video Large Language Models (Video-LLMs) achieve strong performance in video understanding, but their excessive visual tokens bring substantial computational overhead. Existing training-free compression methods improve inference efficiency by reducing visual tokens, yet they often rely on local adjacent-frame similarity for temporal redundancy estimation or allocate token budgets mainly according to segment length. Such designs are sensitive to frame-level noise and fail to capture the non-uniform information distribution of real-world videos. To address these challenges, we propose InfoMerge, a training-free visual token compression method that improves token utilization through robust redundancy estimation and content-aware budget allocation. Specifically, we propose the Temporal Fingerprint Difference: a segment-level second-order temporal redundancy estimation strategy, which models the temporal similarity structure of tokens at the same spatial positions within each segment. We further introduce Content-Aware Budget Allocation (CABA), which dynamically allocates segment-level token budgets based on segment uniqueness and spectral-entropy-based representational richness. By reducing repeated preservation of redundant static regions and allocating more tokens to informative segments, InfoMerge makes better use of the limited token budget while maintaining strong performance. Extensive experiments show that InfoMerge achieves strong efficiency--accuracy trade-offs across multiple benchmarks and backbones, with more pronounced advantages under aggressive compression. On LLaVA-OneVision-7B, InfoMerge retains 98.8\% of the original average performance while reducing 85\% of visual tokens and achieving a 4.24-fold speedup in the prefill stage.

==> latex/section/experiment.tex <==
% \input{latex/table/compar1}
\input{latex/table/3bench}
\input{latex/table/xiaorong1}
% \input{latex/table/tempXiaorong}
% \input{latex/table/chengfa}
% \input{latex/table/wendu}
\input{latex/table/multibench}
\input{latex/table/llavavideo}
\begin{table}[t]
\centering
\caption{Efficiency comparison following MMG-Vid Table 2. Prefill and generate times are measured on LLM decoder forwards only, excluding vision encoding and pruning overhead.}
\label{tab:table2-phase-latency}
	\resizebox{0.97\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{Prefill Time (ms)} & \textbf{Generate Time (ms)} & \textbf{Samples} \\
\midrule
LLaVA-OV & 1505.7 (1.00x) & 32.8 (1.00x) & 30 \\
Ours $r{=}5\%$ & 121.1 (12.43x) & 29.2 (1.12x) & 30 \\
Ours $r{=}7.5\%$ & 152.7 (9.86x) & 27.5 (1.19x) & 30 \\
Pruned $r{=}20\%$ & 323.0 (4.66x) & 29.1 (1.13x) & 30 \\
\bottomrule
\end{tabular}}
\end{table}

\input{latex/table/prefill}

\subsection{Experimental Settings}
\label{sec:exp_setup}

\paragraph{Evaluation Datasets.}
To evaluate the effectiveness of our method across different video understanding scenarios, we conduct experiments on several widely used multimodal video understanding benchmarks, including VideoMME~\cite{fu2025videomme}, MVBench~\cite{li2024mvbench},  MLVU~\cite{zhou2025mlvu}, and LongVideoBench~\cite{wu2024longvideobench}.
% VideoMME covers short-, medium-, and long-duration videos, providing a comprehensive evaluation of multi-scale temporal video question answering.
% MVBench mainly consists of short-video understanding tasks and evaluates the model's ability to understand actions, events, temporal relations, and scene transitions.
% EgoSchema focuses on long-form egocentric videos and emphasizes long-range event reasoning from a first-person perspective.
% MLVU contains diverse video understanding tasks and further evaluates the generalization ability of the method in complex video semantic scenarios.
On LLaVA-OneVision-7B~\cite{li2024llava-ov}, we report full results on all five datasets.
To further verify the cross-backbone generalization ability of our method, we also evaluate LLaVA-Video-7B~\cite{zhang2024llava-video} on two representative benchmarks, VideoMME~\cite{fu2025videomme}.

\paragraph{Baselines.}
We use LLaVA-OneVision-7B~\cite{li2024llava-ov} as the main evaluation backbone and regard the original uncompressed model as the upper-bound baseline.
We compare our method with three training-free visual token compression methods:
1) FastV~\cite{chen2024image}, which prunes visual tokens inside the LLM;
2) VisionZip~\cite{yang2025visionzip}, which performs spatial token compression;
and 3) FastVID~\cite{yang2025visionzip}, which is the baseline method improved in this work.
In addition, to verify that our method is not limited to a single Video-LLM architecture, we further transfer it to LLaVA-Video-7B~\cite{zhang2024llava-video} for comparison.

\paragraph{Implementation Details.}
All evaluations are conducted using LMMS-Eval~\cite{li2024xinrun,zhang2025lmms}.
For LLaVA-OneVision-7B~\cite{li2024llava-ov}, the model samples 32 frames by default.
Each frame is processed by the vision encoder and projector, producing 196 visual tokens per frame.
Therefore, an uncompressed video sample contains up to 6272 visual tokens.
For LLaVA-Video-7B~\cite{zhang2024llava-video}, the model samples 64 frames by default.
All experiments are  conducted on two NVIDIA V100 GPUs.
To systematically evaluate the performance under different compression strengths, we set the visual token retention ratios to 5\%, 10\%, and 15\%.

\subsection{Main Results.}
\textbf{Best performance.}
As shown in Table~\ref{tab:main_results}, our method consistently achieves the best performance under all settings.
At a 10\% retention ratio, FastV and VisionZip suffer performance drops of 10.7\% and 10.1\%, respectively, due to their limited ability to compress temporally redundant tokens.
In contrast, our method preserves 97.8\% of the original performance.
With the proposed improved strategy, even when the retention ratio is reduced to 5\%, our method still retains 93.3\% of the original performance, outperforming FastVID, which preserves 91.5\%.
Meanwhile, the inference computational cost is reduced to ?5.4\%.
These results demonstrate that our method can stably identify temporally redundant tokens and dynamically allocate more token budgets to more informative segments, thereby maintaining strong video understanding ability even under extreme compression.

\textbf{Different Backbones.}
Our method is designed as a plug-and-play module,demonstrates strong cross-backbone transferability.
As shown in Table~\ref{tab:llava_video_results}, our method also shows consistent performance improvement on LLaVA-Video-7B.
At a 10\% retention ratio, it achieves a computational complexity of ? TFLOPs.
This performance surpasses that of LLaVA-OneVision-7B under the 32-frame sampling setting.
These results indicate that our method is effective in extending the input frame length under low token retention ratios, thereby enhancing the model's video understanding capability.

\subsection{Ablation Studies.}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{latex/figures/plot_temp.png}
    \caption{Ablation on temperature}
    \label{fig:temp}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{latex/figures/plot_pen.pdf}
    \caption{Ablation on penalty.}
    \label{fig:pen}
\end{figure}
\textbf{Temporal fingerprint difference.}
Our ablation study confirms the effectiveness of using temporal fingerprint differences to identify temporally redundant tokens.
As shown in Table~\ref{tab:temporal_fingerprint_ablation}, adding the temporal fingerprint difference module to the original FastVID significantly improves the performance.

\input{latex/table/madd-3factor-abla}

\textbf{Two-factor dynamic budget allocation.}
To evaluate the effectiveness of dynamic budget allocation, we conduct the following ablation studies.
First, we fix the overall visual token retention ratio to 10\% and scan the fusion weights of the semantic uniqueness factor and the information density factor.
Specifically, we compare three types of settings: using only semantic uniqueness, using only information density, and fusing the two factors with different weight combinations.
This experiment is designed to verify two aspects:
on the one hand, it analyzes the relative importance of semantic uniqueness and information density in dynamic budget allocation;
on the other hand, it examines whether information density can serve as a complementary factor to further improve segment-level token allocation.
As shown in Table~\ref{tab:two_factor_ablation}, both single-factor settings based on semantic uniqueness or information density improve over the original FastVID, while the two-factor fusion setting further enhances model performance.

\paragraph{Evidence-aware budget allocation.}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{latex/figures/evidence_budget_case.pdf}
    \caption{...}
    \label{fig:evidence_budget_case}
\end{figure}

Figure~\ref{fig:evidence_budget_case} provides a qualitative example of segment-level budget allocation.
The question asks which ingredient is not used, requiring the model to verify the ingredients that actually appear in the video.
The highlighted segment $s_2$ contains colorful thread-like materials, providing evidence that wool thread is used rather than leftover cloth.
Compared with FastVID's length-based allocation, InfoMerge assigns more context-token budget to this segment, which also has higher semantic uniqueness and representational richness.
This suggests that information-density-aware allocation helps preserve task-relevant evidence under limited token budgets.

We further conduct an ablation study on the temperature parameter $\tau$ in dynamic budget allocation.
The temperature controls the sensitivity of the sigmoid modulation function to the segment score $M_k$.
A smaller $\tau$ makes the budget differences among segments smoother, whereas a larger $\tau$ amplifies the differences among segment scores and concentrates the token budget on a few high-scoring segments.
By comparing different $\tau$ values on VideoMME, we evaluate the trade-off between smooth and aggressive budget allocation.
Unless otherwise specified, all ablation studies are conducted on LLaVA-OneVision-7B, using the same frame sampling strategy, inference parameters, and evaluation protocol.

==> latex/section/experiment_change1.tex <==
% \input{latex/table/compar1}
\input{latex/table/3bench}
\input{latex/table/xiaorong1}
% \input{latex/table/tempXiaorong}
% \input{latex/table/chengfa}
% \input{latex/table/wendu}
\input{latex/table/multibench}
\input{latex/table/llavavideo}
\begin{table}[t]
\centering
\caption{Efficiency comparison following MMG-Vid Table 2. Prefill and generate times are measured on LLM decoder forwards only, excluding vision encoding and pruning overhead.}
\label{tab:table2-phase-latency}
	\resizebox{0.97\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{Prefill Time (ms)} & \textbf{Generate Time (ms)} & \textbf{Samples} \\
\midrule
LLaVA-OV & 1505.7 (1.00x) & 32.8 (1.00x) & 30 \\
Ours $r{=}5\%$ & 121.1 (12.43x) & 29.2 (1.12x) & 30 \\
Ours $r{=}7.5\%$ & 152.7 (9.86x) & 27.5 (1.19x) & 30 \\
Pruned $r{=}20\%$ & 323.0 (4.66x) & 29.1 (1.13x) & 30 \\
\bottomrule
\end{tabular}}
\end{table}

\input{latex/table/prefill}
\subsection{Experimental Settings}
\label{sec:exp_setup}

\paragraph{Benchmarks and Baselines.}
We evaluate our method with LMMS-Eval~\cite{li2024xinrun,zhang2025lmms} on four widely used video understanding benchmarks: VideoMME~\cite{fu2025videomme}, MVBench~\cite{li2024mvbench}, MLVU~\cite{zhou2025mlvu}, and LongVideoBench~\cite{wu2024longvideobench}.
LLaVA-OneVision-7B~\cite{li2024llava-ov} is used as the main evaluation backbone, and the original uncompressed model serves as the upper-bound baseline.
We compare our method with representative training-free visual token compression methods, including FastV~\cite{chen2024image}, VisionZip~\cite{yang2025visionzip}, and FastVID~\cite{shen2026fastvid}.
To evaluate cross-backbone generalization, we further transfer our method to LLaVA-Video-7B~\cite{zhang2024llava-video} and report results on VideoMME.

\paragraph{Implementation Details.}
For LLaVA-OneVision-7B, we follow the default setting and sample 32 frames per video.
Each frame is processed into 196 visual tokens, resulting in 6,272 visual tokens for an uncompressed video.
For LLaVA-Video-7B, we sample 64 frames by default.
All experiments are conducted on two NVIDIA V100 GPUs.
We evaluate different compression strengths by setting the visual token retention ratios to 5\%, 10\%, and 15\%.

\subsection{Main Results.}
\textbf{Best performance.}
As shown in Table~\ref{tab:main_results}, our method consistently achieves the best performance under all settings.
At a 10\% retention ratio, FastV and VisionZip suffer performance drops of 10.7\% and 10.1\%, respectively, due to their limited ability to compress temporally redundant tokens.
In contrast, our method preserves 97.8\% of the original performance.
With the proposed improved strategy, even when the retention ratio is reduced to 5\%, our method still retains 93.3\% of the original performance, outperforming FastVID, which preserves 91.5\%.
Meanwhile, the inference computational cost is reduced to ?5.4\%.
These results demonstrate that our method can stably identify temporally redundant tokens and dynamically allocate more token budgets to more informative segments, thereby maintaining strong video understanding ability even under extreme compression.

\textbf{Different Backbones.}
Our method is designed as a plug-and-play module,demonstrates strong cross-backbone transferability.
As shown in Table~\ref{tab:llava_video_results}, our method also shows consistent performance improvement on LLaVA-Video-7B.
At a 10\% retention ratio, it achieves a computational complexity of ? TFLOPs.
This performance surpasses that of LLaVA-OneVision-7B under the 32-frame sampling setting.
These results indicate that our method is effective in extending the input frame length under low token retention ratios, thereby enhancing the model's video understanding capability.

\subsection{Ablation Studies.}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{latex/figures/plot_temp.png}
    \caption{Ablation on temperature}
    \label{fig:temp}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{latex/figures/plot_pen.pdf}
    \caption{Ablation on penalty.}
    \label{fig:pen}
\end{figure}
\textbf{Temporal fingerprint difference.}
Our ablation study confirms the effectiveness of using temporal fingerprint differences to identify temporally redundant tokens.
As shown in Table~\ref{tab:temporal_fingerprint_ablation}, adding the temporal fingerprint difference module to the original FastVID significantly improves the performance.

\input{latex/table/madd-3factor-abla}
\input{latex/table/adj}
\textbf{Two-factor dynamic budget allocation.}
To evaluate the effectiveness of dynamic budget allocation, we conduct the following ablation studies.
First, we fix the overall visual token retention ratio to 10\% and scan the fusion weights of the semantic uniqueness factor and the information density factor.
Specifically, we compare three types of settings: using only semantic uniqueness, using only information density, and fusing the two factors with different weight combinations.
This experiment is designed to verify two aspects:
on the one hand, it analyzes the relative importance of semantic uniqueness and information density in dynamic budget allocation;
on the other hand, it examines whether information density can serve as a complementary factor to further improve segment-level token allocation.
As shown in Table~\ref{tab:two_factor_ablation}, both single-factor settings based on semantic uniqueness or information density improve over the original FastVID, while the two-factor fusion setting further enhances model performance.

\paragraph{Evidence-aware budget allocation.}

\begin{figure}[t]
    \centering
    \includegraphics[
        width=\linewidth,
        trim=90 0 30 0,
        clip
    ]{latex/figures/evidence_budget_case.pdf}
    \caption{Case study of evidence-aware budget allocation.}
    \label{fig:evidence_budget_case}
\end{figure}

Figure~\ref{fig:evidence_budget_case} provides a qualitative example of segment-level budget allocation.
The question asks which ingredient is not used, requiring the model to verify the ingredients that actually appear in the video.
The highlighted segment $s_2$ contains colorful thread-like materials, providing evidence that wool thread is used rather than leftover cloth.
Compared with FastVID's length-based allocation, InfoMerge assigns more context-token budget to this segment, which also has higher semantic uniqueness and representational richness.
This suggests that information-density-aware allocation helps preserve task-relevant evidence under limited token budgets.

We further conduct an ablation study on the temperature parameter $\tau$ in dynamic budget allocation.
The temperature controls the sensitivity of the sigmoid modulation function to the segment score $M_k$.
A smaller $\tau$ makes the budget differences among segments smoother, whereas a larger $\tau$ amplifies the differences among segment scores and concentrates the token budget on a few high-scoring segments.
By comparing different $\tau$ values on VideoMME, we evaluate the trade-off between smooth and aggressive budget allocation.
Unless otherwise specified, all ablation studies are conducted on LLaVA-OneVision-7B, using the same frame sampling strategy, inference parameters, and evaluation protocol.

==> latex/section/intro.tex <==



















Video large language models have demonstrated excellent performance in complex video understanding tasks~\cite{li2024llava-ov,bai2025qwen3,li2025videochat,cheng2024videollama,wang2024qwen2,zhang2024llava-video}. However, their practical deployment is limited by high computational cost and large resource requirements. The bottleneck mainly comes from the quadratic complexity of the attention mechanism and the linear growth of video tokens with video length. For videos containing a large number of frames, the number of tokens can easily reach tens of thousands, making the inference process computationally expensive. For example,  in LLaVA-OV-7B~\cite{li2024llava-ov}, 196 tokens are retained for a single video frame. Therefore, a 32-frame video will accumulate 6272 tokens, among which many tokens are highly redundant and may even act as noise that interferes with the reasoning of the LLM.

Token compression is a promising research direction. Current training-free video token compression methods mainly follow several routes:(1)Pruning along the spatial dimension and retaining tokens with high saliency, such as attention-based methods ,such as VisionZip~\cite{yang2025visionzip} and FastV~\cite{chen2024image}.
(2)Identifying temporally redundant tokens, usually by using the cosine similarity between tokens at the same spatial location in adjacent frames, such as DyCoke~\cite{tao2025dycoke}.
(3)Staged spatio-temporal methods. These methods perform compression along the temporal and spatial dimensions respectively, such as FastVID~\cite{shen2026fastvid} and HoliTom~\cite{shao2025holitom}. The default assumption of these methods is spatio-temporal separability, but recent studies have found that under extremely low retention rates, this assumption often does not hold.
(4)Unified spatio-temporal compression, such as USTC~\cite{du2026unified}, D²Pruner~\cite{zhang2026d2pruner}, and MMG-Vid~\cite{ma2026mmg}?

We first ask: why can video tokens be compressed?
We conduct experiments from the perspective of representation space.
By performing SVD analysis on the token set in the pruning candidate region, we find that its singular value spectrum decays rapidly: the effective rank (eRank)~\cite{roy2007effective} converted from normalized spectral entropy is far smaller than the theoretical upper bound.
This indicates that token representations are not uniformly distributed in the high-dimensional space, but are concentrated on a small number of dominant directions.
Such local low-rank collapse explains the compressibility of video tokens, and further suggests that relying solely on pairwise cosine similarity for redundancy identificatio) is susceptible to local perturbations and ranking instability.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{latex/figures/intro_low_rank_collapse.png}
    \caption{ Singular value spectra of video token representations in pruning candidate regions.
    The spectral energy decays rapidly across different video segments, and the effective rank is much smaller than the full-rank upper bound.
    This indicates a local low-rank collapse of video tokens, providing empirical evidence for their compressibility.
}
    \label{fig:low-erank}
\end{figure}

However,existing methods generally rely on a local metric when identifying temporal redundancy: comparing the feature similarity of tokens at the same spatial location in adjacent frames~\cite{tao2025dycoke,shao2025holitom}. This design implies an assumption that the same spatial location has a stable semantic correspondence between adjacent frames, and that its feature distance can reliably reflect semantic changes. However, in real videos, this assumption often does not hold. Slight camera shake, local viewpoint shift, video compression noise, and object boundary displacement may all cause significant fluctuations in token features at the same spatial location. As a result, static backgrounds may be misjudged as significant changes, while locations with real semantic changes may also be mistakenly pruned due to accidental similarity in local features. As shown in Figure~\ref{fig:low-erank}, temporal redundancy estimation directly based on raw token distance shows obvious instability under changes in frame distance.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{latex/figures/tokenchose.png}
    \caption{
Qualitative comparison of token selection on VideoMME under 10\% retention.
For the question ``Why does the roof object fly?'', the ground-truth answer is ``Lunar approach''.
Original FastVID predicts ``There was an explosion'', while our method predicts the correct answer.
Blue boxes denote tokens selected only by our method, and red boxes denote tokens selected only by FastVID.
Compared with FastVID, our method retains more temporally informative visual evidence associated with the lunar approach and the flying roof object.
}
    \label{fig:tokenchose}
\end{figure}

In addition, methods such as FastVID~\cite{shen2026fastvid} use static token budget allocation, that is, the original budget allocation usually statically assigns the number of tokens according to segment length. This practice implies a strong assumption: the longer the segment, the more tokens it deserves to retain. However, the amount of information in a video does not grow linearly with the number of frames, which ultimately limits the preservation of effective information during compression, as shown in Figure~\ref{fig:tokenchose} where FastVID gives an incorrect answer.

We reformulate the video token compression problem as a segment-level spatio-temporal redundancy fusion problem under ranking stability constraints, aiming to provide a budget allocation scheme that is robust to low-rank collapse, preserve truly non-spatio-temporally redundant tokens, and dynamically allocate token budgets according to segment content. Different from previous methods that compare cosine similarity between tokens at the same spatial location in adjacent frames, we propose to stably identify truly redundant tokens in noisy environments based on temporal fingerprint differences. Meanwhile, we design a dynamic token allocation scheme based on uniqueness and information density, and introduce text awareness. To this end, we design a selection module. This module first divides the video into semantically consistent segments, then performs stable temporal redundancy identification for tokens at each spatial location within each segment, and further dynamically allocates token budgets according to segment uniqueness reflected by inter-segment mean feature distance and local density reflected by spectral entropy.  The whole module is training-free and plug-and-play, and can be flexibly integrated into existing VLLMs. Meanwhile, our temporal fingerprint difference-based spatio-temporal redundancy perception can easily replace the similarity-based redundancy identification modules in existing methods. For example, as shown in the figure/table, when we replace the temporal redundancy identification method in HoliTom with ours, the accuracy on VideoMME is improved.

Experimental evaluation verifies the effectiveness of our proposed method in achieving an ideal efficiency-performance trade-off. Specifically, as shown in Figure ?, on the LLaVA-OneVision-7B model~\cite{li2024llava-ov}, the computational cost is reduced to only ??\% of the original FLOPs, while ??\% of the original model performance is well preserved. In addition, we observe a significant improvement in inference efficiency, with TTFT shortened to ??\% of the original. Compared with the original FastVID, our method achieves excellent improvements in both performance and efficiency. Meanwhile, our method shows strong generalization ability across various VLLM architectures, demonstrating its excellent generality and deployment convenience.

Our contributions are summarized as follows:
\begin{itemize}
    \item Through experiments, we find low rank in the high-dimensional space, which is the reason why VLLMs can perform token compression and also the motivation for designing a stable redundancy identification method.
    \item We use segment-level temporal fingerprint differences to identify temporal redundancy, so as to preserve truly useful information.
    \item Under extremely low retention rates, our method can still significantly improve efficiency while maintaining most of the original performance, achieving state-of-the-art performance.
    \item We design the whole module to be training-free and plug-and-play, ensuring that it can be flexibly integrated into existing VLLMs.
\end{itemize}


==> latex/section/intro_change1.tex <==

Video Large Language Models (VLLMs) have recently achieved remarkable progress in complex video understanding tasks~\cite{li2024llava-ov,bai2025qwen3,li2025videochat,cheng2024videollama,wang2024qwen2,zhang2024llava-video}. Despite their strong capabilities, their practical deployment remains severely constrained by the high computational and memory costs induced by video tokens. This issue is primarily attributed to the quadratic complexity of attention and the linear growth of token sequences with video length.
% For instance, in LLaVA-OV-7B~\cite{li2024llava-ov}, each frame is represented by 196 visual tokens, resulting in over 6K tokens for a 32-frame video, many of which are highly redundant or even detrimental to reasoning.

Token compression has therefore emerged as a key direction for efficient VLLM inference. Existing training-free methods can be broadly categorized into spatial pruning methods~\cite{yang2025visionzip,chen2024image}, temporal redundancy reduction methods~\cite{tao2025dycoke}, staged spatio-temporal compression methods~\cite{shen2026fastvid,shao2025holitom}, and unified spatio-temporal approaches~\cite{du2026unified,zhang2026d2pruner,ma2026mmg}. Despite their progress, most existing methods rely on a common underlying assumption: \textit{local pairwise similarity is sufficient to characterize redundancy}. In practice, however, this assumption becomes fragile under real-world video noise, motion, and viewpoint variations, leading to unstable redundancy estimation and suboptimal token allocation.

In this work, we argue that video token redundancy should be understood from a more structured perspective rather than local similarity. Our key observation is that visual token representations exhibit \textbf{segment-wise low-rank structure}, where information is concentrated along a few dominant directions within each temporal segment. We empirically verify this by performing singular value decomposition on candidate token representations, showing that the effective rank is significantly smaller than the full dimensionality. This low-rank property explains why video tokens are compressible, but also reveals a critical limitation: redundancy cannot be reliably captured by local pairwise similarity alone, as it is inherently a global structural property rather than a point-wise metric.


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{latex/figures/tokenchose.png}
%     \caption{
% Qualitative comparison of token selection on VideoMME under 10\% retention.
% For the question ``Why does the roof object fly?'', the ground-truth answer is ``Lunar approach''.
% Original FastVID predicts ``There was an explosion'', while our method predicts the correct answer.
% Blue boxes denote tokens selected only by our method, and red boxes denote tokens selected only by FastVID.
% Compared with FastVID, our method retains more temporally informative visual evidence associated with the lunar approach and the flying roof object.
% }
%     \label{fig:tokenchose}
% \end{figure}
\begin{figure*}[t]
    \centering
    \includegraphics[
        width=\linewidth,
        trim=15 105 10 25,
        clip
    ]{latex/figures/token_selection_comparison_figure_style.pdf}
    \caption{Qualitative generation comparison between our method and other approaches.
}
    \label{fig:tokenchose}
\end{figure*}



Building on this insight, we further identify two key challenges in existing methods. First, local similarity-based redundancy estimation is highly sensitive to noise, such as camera jitter, compression artifacts, and small spatial shifts, which leads to inconsistent identification of static and dynamic tokens. Second, most methods adopt a heuristic token allocation strategy based on segment length, implicitly assuming that longer segments contain more information, which is often violated in real-world videos where information density varies significantly across time.

To address these limitations, we propose \textbf{InfoMerge}, a training-free framework that rethinks video token compression from a segment-structured redundancy perspective. Instead of directly measuring first-order feature differences between adjacent frames, we introduce a \textbf{Temporal Fingerprint Difference (TFD)} module, {\color{red}which captures second-order temporal consistency by comparing pairwise similarity fingerprints over time within each segment. This enables more robust identification of truly redundant tokens under noisy conditions.}

Furthermore, to address the mismatch between token budget and information distribution, we propose an \textbf{Content-Aware Budget Allocation (CABA)} strategy. CABA jointly considers segment-level uniqueness and internal representation complexity, enabling adaptive allocation of token budgets according to both semantic distinctiveness and {\color{red}representational richness}.

{\color{red}Finally, guided by the temporal redundancy prior from TFD and the segment-wise budget allocation from CABA, we build a unified spatio-temporal compression pipeline that jointly performs redundancy-aware token pruning and merging in a training-free and plug-and-play manner.}

Extensive experiments demonstrate that InfoMerge achieves a superior efficiency–accuracy trade-off. It consistently improves performance under aggressive token compression ratios while significantly reducing computational cost. In addition, the proposed method generalizes well across different VLLM architectures, demonstrating its effectiveness and robustness for efficient video understanding.
Our contributions are summarized as follows:
\begin{itemize}
    \item We identify that video tokens exhibit segment-wise low-rank structure, revealing that redundancy is fundamentally a global structural property rather than a local similarity phenomenon.
    \item We propose Temporal Fingerprint Difference (TFD), a robust redundancy estimation method that captures stable temporal consistency beyond noisy frame-wise similarity.
    \item We introduce Information-Density-Aware Budget Allocation (CABA), which dynamically allocates token budgets based on both semantic uniqueness and {\color{red}representational richness}.
    \item We design a training-free, plug-and-play compression framework that significantly improves efficiency–performance trade-offs and generalizes across VLLM architectures.
\end{itemize}
 


==> latex/section/intro_gsw.tex <==
Video LLMs have achieved remarkable progress in complex video understanding tasks~\cite{li2024llava-ov,bai2025qwen3,li2025videochat,cheng2024videollama,wang2024qwen2,zhang2024llava-video}. Despite their strong capabilities, their practical deployment remains severely constrained by the high computational and memory costs induced by video tokens. This issue is primarily attributed to the quadratic complexity of attention and the linear growth of token sequences with video length. 

Token compression has therefore emerged as a key direction for efficient Video LLM inference. Existing training-free methods can be broadly categorized into spatial pruning methods~\cite{yang2025visionzip,chen2024image}, temporal redundancy reduction methods~\cite{tao2025dycoke}, staged spatio-temporal compression methods~\cite{shen2026fastvid,shao2025holitom}, and unified spatio-temporal approaches~\cite{du2026unified,zhang2026d2pruner}. Despite their progress, most existing methods rely on a common underlying assumption: \textit{local pairwise similarity is sufficient to characterize redundancy}. In practice, however, this assumption becomes fragile under real-world video noise, motion, and viewpoint variations, leading to unstable redundancy estimation and suboptimal token allocation.

In this work, we argue that video token redundancy should be understood from a more structured perspective rather than local similarity. Our key observation is that visual token representations exhibit \textbf{segment-wise low-rank structure}, where information is concentrated along a few dominant directions within each temporal segment. We empirically verify this by performing singular value decomposition on candidate token representations, showing that the effective rank is significantly smaller than the full dimensionality. This low-rank property explains why video tokens are compressible, but also reveals a critical limitation: redundancy cannot be reliably captured by local pairwise similarity alone, as it is inherently a global structural property rather than a point-wise metric.


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{latex/figures/tokenchose.png}
%     \vspace{-3mm}
% \caption{ Qualitative comparison of token selection.
% Compared with FastVID, our method preserves more temporally informative regions related to the flying roof object, leading to the correct prediction.
% Blue boxes indicate tokens selected only by our method, and red boxes indicate tokens selected only by FastVID.
% }
%     \label{fig:tokenchose}
%      \vspace{-3mm}
% \end{figure}
\begin{figure*}[t]
    \centering
    \includegraphics[
        width=\linewidth,
        trim=15 105 10 25,
        clip
    ]{latex/figures/token_selection_comparison_figure_style.pdf}
    \caption{Qualitative generation comparison between our method and other approaches.
}
    \label{fig:tokenchose}
\end{figure*}

%    \caption{ Qualitative comparison of token selection on VideoMME under 10\% retention. For the question ``Why does the roof object fly?'', the ground-truth answer is ``Lunar approach''. Original FastVID predicts ``There was an explosion'', while our method predicts the correct answer. Blue boxes denote tokens selected only by our method, and red boxes denote tokens selected only by FastVID. Compared with FastVID, our method retains more temporally informative visual evidence associated with the lunar approach and the flying roof object. }


Building on this insight, we further identify two key challenges in existing methods. First, local similarity-based redundancy estimation is highly sensitive to noise, such as camera jitter, compression artifacts, and small spatial shifts, which leads to inconsistent identification of static and dynamic tokens. Second, most methods adopt a heuristic token allocation strategy based on segment length, implicitly assuming that longer segments contain more information, which is often violated in real-world videos where information density varies significantly across time.

To address these limitations, we propose \textbf{InfoMerge}, a training-free framework that rethinks video token compression from a segment-structured redundancy perspective. Instead of relying on local similarity, we introduce a \textbf{Temporal Fingerprint Difference (TFD)} module, which captures stable temporal consistency patterns at each spatial position within a segment by modeling pairwise similarity structures over time. This enables more robust identification of truly redundant tokens under noisy conditions.
Furthermore, to address the mismatch between token budget and information distribution, we propose an \textbf{Information-Density-Aware Budget Allocation (IDAB)} strategy. IDAB jointly considers segment-level uniqueness and internal representation complexity, enabling adaptive allocation of token budgets according to both semantic distinctiveness and spectral information density.
Finally, we integrate TFD and IDAB into a unified spatio-temporal compression pipeline that performs redundancy-aware token pruning and merging in a training-free and plug-and-play manner. The proposed framework can be seamlessly integrated into existing VLLMs and directly replaces similarity-based redundancy modules in prior methods.
Extensive experiments demonstrate that InfoMerge achieves a superior efficiency–accuracy trade-off.
Our contributions are summarized as follows:

\iffalse
\begin{itemize}
    \item We identify that video tokens exhibit segment-wise low-rank structure, revealing that redundancy is fundamentally a global structural property rather than a local similarity phenomenon.
    \item We propose Temporal Fingerprint Difference module, a robust redundancy estimation method that captures stable temporal consistency beyond noisy frame-wise similarity.
    \item We introduce Information-Density-Aware Budget Allocation strategy, which dynamically allocates token budgets based on both semantic uniqueness and representation complexity.
    \item We design a training-free, plug-and-play compression framework that significantly improves efficiency–performance trade-offs and generalizes across VLLM architectures.
\end{itemize}
\fi

 
\begin{itemize}
    \item We show that video tokens exhibit segment-wise low-rank structure, revealing that redundancy is fundamentally a global structural property rather than a local similarity phenomenon. Based on this observation, we develop a training-free and plug-and-play compression strategy that achieves strong efficiency--performance trade-offs across diverse Video LLMs.
    
    \item We propose Temporal Fingerprint Difference, a robust redundancy estimation method that captures stable temporal consistency beyond noisy frame-wise similarity, enabling more reliable identification of redundant  tokens.
    
    \item We introduce an Information-Density-Aware Budget Allocation strategy that dynamically allocates token budgets according to both semantic uniqueness and representation complexity, improving token utilization under extremely low retention rates.
\end{itemize}

==> latex/section/method.tex <==

\subsection{Overview}
\label{sec:method:overview}

As illustrated in Fig.~\ref{fig:method}, our method follows the overall pipeline of FastVID.
Given an input video, we first apply Dynamic Temporal Segmentation (DySeg) to divide the sampled frames into temporally ordered and internally coherent segments.
Then, spatio-temporal token compression is performed within each segment.
Different from FastVID, InfoCarve redesigns two key components.

First, we introduce a temporal fingerprint difference to estimate the temporal stability of each spatial position within a segment.
Instead of only comparing adjacent frames, we construct a segment-level pairwise similarity fingerprint for each spatial position and measure its temporal variation by the mean absolute difference of the fingerprint matrix.
This component is detailed in Sec.~\ref{sec:method:madd}.

Second, we propose an information-density-aware budget allocation strategy.
By jointly considering segment uniqueness and segment information density, InfoCarve adaptively allocates the limited context-token budget to different segments.
This component is detailed in Sec.~\ref{sec:method:budget}.

Formally, suppose the sampled video contains $F$ frames.
After the visual encoder, projector, and pooling operation, each frame contains $T$ visual tokens with hidden dimension $D$.
We denote the visual features of the whole video as
$\mathbf{H}\in\mathbb{R}^{F\times T\times D}$, where
$\mathbf{H}_{f,p}\in\mathbb{R}^{D}$ represents the token at the $p$-th spatial position of the $f$-th frame.
The frame-level global feature is denoted as $\mathbf{g}_f\in\mathbb{R}^{D}$.
Based on the retention ratio $r$, we compute the number of ATS tokens per frame, denoted as $T_s$, and the initial average number of DTM context tokens per frame, denoted as $T_c$.

\subsection{DySeg}
\label{sec:method:dyseg}

We first perform dynamic temporal segmentation on the sampled video frames.
DySeg adaptively determines segment boundaries according to the semantic transition strength between adjacent frames.

Specifically, for the global features $\mathbf{g}_f$ and $\mathbf{g}_{f+1}$ of two adjacent frames, we compute their transition similarity as:
\begin{equation}
s_f = \cos(\mathbf{g}_f,\mathbf{g}_{f+1}),
\quad f=1,\dots,F-1,
\end{equation}
where $F$ denotes the number of sampled frames, and $s_f$ denotes the transition similarity between the $f$-th frame and the $(f+1)$-th frame.
A lower $s_f$ indicates a stronger semantic transition between two adjacent frames, and is therefore more suitable as a segment boundary.
We denote all transition similarities as
$\mathcal{T}=\{s_f\}_{f=1}^{F-1}$.

We use both the minimum number of segments $c$ and the similarity threshold $\tau_{\mathrm{seg}}$ to control the segmentation granularity.
The candidate boundaries consist of two parts:
\begin{equation}
\mathcal{S}_1 = \operatorname{argmin}_{c-1} \mathcal{T},
\quad

\mathcal{S}_2 = \{ f \mid s_f < \tau_{\mathrm{seg}},\ s_f \in \mathcal{T} \},
\quad

\mathcal{S} = \mathcal{S}_1 \cup \mathcal{S}_2 .
\end{equation}

Here, $\mathcal{S}_1$ denotes the $c-1$ transition positions with the lowest similarity, which ensures that the video is divided into at least $c$ segments.
$\mathcal{S}_2$ denotes all transition positions whose similarity is below the threshold $\tau_{\mathrm{seg}}$, which captures obvious semantic changes.
Each position in $\mathcal{S}$ is treated as a segment boundary.

This design can adapt to both simple and complex videos.
For videos with few shot changes, $\mathcal{S}_2$ may be empty, while $\mathcal{S}_1$ can still provide fine-grained segmentation according to relatively weaker transition similarities.
For complex videos with obvious scene changes or motion transitions, $\mathcal{S}_2$ directly captures low-similarity transitions and separates adjacent frames with clear semantic changes into different segments.

\subsection{Temporal Fingerprint Difference}
\label{sec:method:madd}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{latex/figures/MADD_editable_diagram.pdf}
    \caption{Illustration of the proposed temporal fingerprint difference. For each spatial position, we first build an intra-segment pairwise similarity matrix over all frames, then compute the frame-wise row differences and average them to obtain the MADD score. A smaller MADD value indicates a more temporally stable position and thus higher temporal redundancy.}
    \label{fig:madd}
\end{figure}

The original FastVID does not explicitly distinguish static tokens from dynamic tokens.
Within each segment, we aim to identify spatial positions that are highly redundant along the temporal dimension.
A common way to estimate temporal redundancy is to compute the cosine similarity between tokens at the same spatial position in adjacent frames.
If $\cos(\mathbf{H}_{f,p},\mathbf{H}_{f+1,p})$ is high, position $p$ is regarded as temporally stable.
However, this criterion only uses local relationships between adjacent frames and is vulnerable to frame-level noise.
Moreover, in high-dimensional visual feature spaces, the absolute differences between cosine similarity values can be small, making it difficult to distinguish static positions from dynamic ones.

To obtain a more robust estimate of temporal redundancy, we propose \textbf{temporal fingerprint difference}, as illustrated in Fig.~\ref{fig:madd}.
Instead of only observing token similarity between adjacent frames, we construct a segment-level pairwise similarity fingerprint for each spatial position.
For spatial position $p$ in segment $\mathcal{V}_k$, we first apply $\ell_2$ normalization to the token representations across all frames:
\begin{equation}
\hat{\mathbf{x}}^{(k)}_{s,p}
=
\frac{
\mathbf{H}^{(k)}_{s,p}
}{
\|\mathbf{H}^{(k)}_{s,p}\|_2
},
\quad s=1,\dots,S_k.
\end{equation}
Then, we construct the temporal similarity fingerprint matrix for position $p$:
\begin{equation}
\mathbf{F}^{(k)}_p[s,s']
=
\left\langle
\hat{\mathbf{x}}^{(k)}_{s,p},
\hat{\mathbf{x}}^{(k)}_{s',p}
\right\rangle,
\quad
s,s'=1,\dots,S_k.
\end{equation}
Here, $\mathbf{F}^{(k)}_p\in\mathbb{R}^{S_k\times S_k}$ describes the global temporal consistency of position $p$ within the entire segment.
If this position corresponds to static background or repeated semantics, its similarity fingerprint should vary only slightly along the temporal dimension.
In contrast, if the position contains moving objects, action changes, or semantic transitions, the similarity distributions of adjacent rows will change more significantly.

Therefore, we compute the first-order difference of the fingerprint matrix along the temporal dimension and take the mean absolute value:
\begin{equation}
\mathrm{MADD}^{(k)}(p)
=
\frac{1}{(S_k-1)S_k}
\sum_{s=1}^{S_k-1}
\sum_{s'=1}^{S_k}
\left|
\mathbf{F}^{(k)}_p[s+1,s']
-
\mathbf{F}^{(k)}_p[s,s']
\right|.
\end{equation}
A smaller MADD value indicates that the spatial position has a more stable pairwise similarity structure within the segment, and is therefore more likely to be temporally redundant.
For each segment, we select the $\lfloor \rho T\rfloor$ spatial positions with the smallest MADD values as the static candidate set:
\begin{equation}
\mathcal{S}^{(k)}
=
\operatorname{Top}_{\lfloor \rho T\rfloor}
\left(-\mathrm{MADD}^{(k)}(p)\right),
\end{equation}
where $\rho$ controls the proportion of spatial positions regarded as static candidates in each segment.

We use the static candidate set as a prior for subsequent compression.
In the ATS branch, we apply a soft penalty to static positions that have already been repeatedly selected.
In the DTM branch, we apply a hard mask to static positions that have already been selected.
In this way, InfoCarve reduces repeated preservation of static tokens without directly discarding them.

\subsection{Information-Density-Aware Budget Allocation}
\label{sec:method:budget}

FastVID allocates the context-token budget to each segment according to segment length.
This allocation strategy ignores the differences in information density across segments.
For example, a long static background segment may contain many frames but only limited new information.
In contrast, a short but action-dense segment may require more context tokens to preserve key visual semantics.

To address this issue, we design an information-density-aware budget allocation mechanism.
For the $k$-th segment, we estimate its information content from two perspectives: segment uniqueness and information density.

\paragraph{Segment Uniqueness.}
We first compute the segment-level average feature:
\begin{equation}
\bar{\mathbf{x}}_k
=
\frac{1}{S_kT}
\sum_{s=1}^{S_k}\sum_{p=1}^{T}
\mathbf{H}^{(k)}_{s,p}.
\end{equation}
Then, we compute the global video feature:
\begin{equation}
\bar{\mathbf{x}}_{\mathrm{glob}}
=
\frac{
\sum_{k=1}^{K} S_k\bar{\mathbf{x}}_k
}{
\sum_{k=1}^{K}S_k
}.
\end{equation}
The segment uniqueness is defined by the cosine distance between the segment feature and the global video feature:
\begin{equation}
u_k
=
1-\cos(\bar{\mathbf{x}}_k,\bar{\mathbf{x}}_{\mathrm{glob}}).
\end{equation}
A larger $u_k$ indicates that the segment is more distinct from the global video semantics and is more likely to contain key information.

\paragraph{Information Density.}
As shown in Fig.~\ref{fig:erank}, low-density segments usually have a smaller effective rank, with their token energy concentrated in only a few principal directions.
For example, a small number of semantic directions can already explain most of the visual information.
In contrast, high-density segments have a larger effective rank and a more uniform energy distribution, indicating richer visual representations.
Therefore, we use spectral entropy to measure segment information density.

For the $k$-th segment, we flatten its tokens into
$\mathbf{X}_k\in\mathbb{R}^{S_kT\times D}$ and compute its singular values
$\{\sigma_j\}_{j=1}^{R}$, where $R=\min(S_kT,D)$.
The normalized squared energy is defined as:
\begin{equation}
\pi_j
=
\frac{\sigma_j^2}{\sum_{\ell=1}^{R}\sigma_\ell^2}.
\end{equation}
Here, $\sigma_j$ denotes the $j$-th singular value, and $R$ denotes the number of singular values used in the computation.
Based on this distribution, we use Shannon entropy to measure how evenly the singular-value energy is distributed, and normalize it as the segment density:
\begin{equation}
e_k
=
\frac{
-\sum_{j=1}^{R}\pi_j\log \pi_j
}{
\log R
}.
\end{equation}
Since $e_k\in[0,1]$, it reflects how dispersed the visual-token energy is across different principal directions.
When $e_k$ is small, the visual representation of the segment is mainly concentrated in a few principal directions, suggesting a relatively simple semantic structure.
When $e_k$ is large, the token energy is more evenly distributed across more principal directions, indicating that the segment contains a more complex semantic structure and is harder to represent with only a few tokens.

Since the two factors have different scales, we first apply z-score normalization across all segments and then linearly combine them:
\begin{equation}
m_k
=
\alpha z(u_k)+\beta z(e_k),
\end{equation}
where $\alpha$ and $\beta$ control the relative weights of the two factors.

We then use a sigmoid function to map the fused score to a smooth budget modulation coefficient and multiply it by the segment length:
\begin{equation}
w_k
=
\sigma(\tau_{\mathrm{bud}}m_k)\cdot S_k.
\end{equation}
Finally, the context-token budget for the $k$-th segment is computed as:
\begin{equation}
B_k
=
\max
\left(
1,
\operatorname{round}
\left(
\frac{F T_c w_k}{\sum_{j=1}^{K}w_j}
\right)
\right).
\end{equation}
As the temperature coefficient $\tau_{\mathrm{bud}}$ increases, the budget is gradually biased toward segments with higher information density.

\subsection{Spatio-Temporal Compression}
\label{sec:method:compression}

After obtaining the static candidate set and the context-token budget, we perform spatio-temporal compression within each segment.
Overall, we retain the two branches of STPrune: ATS selects salient tokens based on attention scores, while DTM preserves contextual tokens.
Different from the original design, our improved ATS and DTM use the static prior obtained from temporal fingerprint difference to reduce repeated selection of static tokens.

\paragraph{Attention-based Token Selection.}
After separating tokens in each segment into dynamic and static candidates, we use the [CLS] attention score from the visual encoder to measure the importance of different visual tokens.
Prior studies have shown that the attention from the [CLS] token to patch tokens can serve as an effective estimate of visual saliency.

However, many Video-LLMs adopt SigLIP as the visual encoder and use its penultimate-layer features as inputs to the subsequent LLM.
Since this pathway omits the SigLIP head, the original [CLS] token and the corresponding [CLS] attention scores cannot be directly obtained.
Following FastVID, we re-attach the pretrained SigLIP head to the visual encoder to compute additional [CLS] attention scores without changing the main representation pathway of the Video-LLM.
Since the SigLIP head is lightweight, this introduces only minor computational overhead compared with the full Video-LLM.

Specifically, for the $f$-th frame, we extract the attention scores from the [CLS] token to spatial visual tokens from the pretrained SigLIP head:
\begin{equation}
\mathbf{A}_f \in \mathbb{R}^{H \times W},
\end{equation}
where $H$ and $W$ denote the spatial dimensions of visual tokens.
Since Video-LLMs usually apply pooling to visual tokens, we apply the same pooling operation to $\mathbf{A}_f$ to align the attention scores with the visual tokens actually passed to the LLM:
\begin{equation}
\bar{\mathbf{A}}_f \in \mathbb{R}^{\bar{H} \times \bar{W}},
\end{equation}
where $\bar{H}$ and $\bar{W}$ denote the pooled spatial dimensions.
Then, for each frame, we select the top-$T_s$ tokens according to the attention scores:
\begin{equation}
\mathcal{T}^{\mathrm{ATS}}_f
=
\operatorname{Top}_{T_s}(\bar{\mathbf{A}}_{f}).
\end{equation}

However, applying ATS independently to each frame may repeatedly select the same static background positions due to their high attention scores.
Although these tokens may contain certain visual information, preserving near-duplicate static regions multiple times within the same segment wastes the limited token budget.
Therefore, we further introduce a soft penalty for repeated static positions on top of the original ATS.

Let $\mathcal{S}^{(k)}$ denote the static candidate set identified in segment $\mathcal{V}_k$, and let $\mathcal{P}^{(k)}_{f-1}$ denote the set of static positions that have been selected by ATS before the $f$-th frame.
For position $p$ in frame $f$, we recompute the pooled attention score as:
\begin{equation}
\tilde{\mathbf{A}}_{f,p}
=
\bar{\mathbf{A}}_{f,p}
-
\lambda \cdot
\operatorname{std}(\bar{\mathbf{A}}_{f})
\cdot
\mathbb{1}
\left[
p \in \mathcal{S}^{(k)}
\land
p \in \mathcal{P}^{(k)}_{f-1}
\right],
\end{equation}
where $\lambda$ is the penalty strength, and
$\operatorname{std}(\bar{\mathbf{A}}_{f})$ adaptively scales the penalty according to the attention distribution of the current frame.
Finally, ATS selects salient tokens from the adjusted attention scores:
\begin{equation}
\mathcal{T}^{\mathrm{ATS}}_f
=
\operatorname{Top}_{T_s}(\tilde{\mathbf{A}}_{f}).
\end{equation}

This penalty is a soft constraint rather than a hard mask.
Therefore, if a previously selected static token still has a sufficiently high attention score, it can still be retained.
In most cases, however, repeated static positions are down-weighted, releasing more token budget for newly emerging dynamic regions or fine-grained visual details.

\paragraph{Hard-masked DTM.}
DTM is used to preserve segment-level contextual information.
For each segment, we select anchor frames at a fixed interval $p$, and select context anchor tokens in each anchor frame using DPC-KNN.
For the $k$-th segment, the number of anchor frames is:
\begin{equation}
n_a^{(k)}=\left\lceil\frac{S_k}{p}\right\rceil.
\end{equation}
Given the dynamic budget $B_k$, the number of context tokens selected in each anchor frame is:
\begin{equation}
T^{(k)}_{c,a}
=
\left\lfloor\frac{B_k}{n_a^{(k)}}\right\rfloor.
\end{equation}

In each anchor frame, we first compute the density score of candidate tokens.
For token $v_i$ in an anchor frame, its local density is defined as:
\begin{equation}
\rho_i
=
\exp
\left(
-\frac{1}{K_{\mathrm{nn}}}
\sum_{v_j\in \mathrm{kNN}(v_i)}
d(v_i,v_j)^2
\right),
\end{equation}
and its nearest distance to a token with higher density is:
\begin{equation}
    \begin{aligned}
    \delta_i =
\min_{j:\rho_j>\rho_i} d(v_i,v_j), & \exists j,\rho_j>\rho_i, \\ 
\max_j d(v_i,v_j), & \text{otherwise}.
    \end{aligned}
\end{equation}
The final density-peak score is $\rho_i\delta_i$.

However, if multiple anchor frames select the same static position as density centers, the context budget will still be consumed by repeated static information.
To address this issue, we introduce a static hard mask into DTM.
Let $\mathcal{Q}^{(k)}_{a-1}$ denote the set of static positions that have already been selected by the previous $a-1$ anchor frames in the current segment.
For the $a$-th anchor frame, if a position $p$ belongs to $\mathcal{Q}^{(k)}_{a-1}$, we set its density-peak score to $-\infty$:
\begin{equation}
\rho_{a,p}\delta_{a,p}
\leftarrow
-\infty,
\quad
p\in \mathcal{Q}^{(k)}_{a-1}.
\end{equation}
Then, we select the top-$T^{(k)}_{c,a}$ context anchors.
Different from the soft penalty used in ATS, the hard mask in DTM directly prevents the same static position from repeatedly becoming a context center across multiple anchor frames, thereby improving the spatial coverage and semantic diversity of context tokens.

\paragraph{Anchor-centric Aggregation.}
After selecting context anchors, each unreserved token within the segment is assigned to its most similar anchor center.
For an anchor token $a$ and its assigned token set $\{b_1,\dots,b_n\}$, the updated anchor representation is:
\begin{equation}
a^\star
=
\mu a
+
(1-\mu)
\frac{1}{n}
\sum_{j=1}^{n}b_j,
\end{equation}
where $\mu$ controls the weight between the original anchor token and the merged tokens.
Since the merged representation is written back to the original position of the anchor token, DTM preserves the positional structure and avoids disrupting the spatio-temporal order of video tokens.

Finally, we concatenate the salient tokens obtained by ATS and the context anchors obtained by DTM from each segment in temporal order.
The resulting compressed video-token sequence is then fed into the LLM together with the text tokens.


==> latex/section/method_gsw.tex <==

\subsection{Overview}
\label{sec:method:overview}
{\color{blue}

\iffalse
As illustrated in Fig.~\ref{fig:method}, following the efficient video processing paradigm of FastV~\cite{fastvid}, we propose \textbf{InfoCarve}, an adaptive token purging framework for efficient video large language models (VLLMs). InfoCarve consists of three key stages. First, we adopt Dynamic Temporal Segmentation (DySeg)~\cite{fastvid} to partition the sampled video frames into temporally ordered and semantically coherent segments. Instead of processing all video tokens uniformly, spatio-temporal token compression is performed independently within each segment, enabling finer-grained modeling of temporal redundancy. Second, we observe that existing FastV-style methods do not explicitly distinguish static tokens from dynamic tokens, leading to inefficient retention of redundant visual content. To address this issue, we propose a \textbf{Temporal Fingerprint Difference (TFD)} module, which estimates temporal variation across frames and identifies dynamically informative regions within each segment. Third, we further observe that different temporal segments often exhibit highly imbalanced information density. Uniform token allocation therefore leads to suboptimal computation distribution. To overcome this limitation, we introduce an \textbf{Information-Density-Aware Budget Allocation (IDAB)} strategy, which dynamically allocates token budgets according to the estimated information density of each segment. Based on the proposed TFD and IDAB modules, InfoCarve progressively purges redundant visual tokens while preserving semantically important spatio-temporal information. The final retained video tokens are then combined with query tokens and fed into the LLM to generate responses efficiently.
\fi


As illustrated in Fig.~\ref{fig:method}, following the efficient video processing paradigm of FastVid~\cite{shen2026fastvid}, we propose \textbf{InfoCarve}, an adaptive token purging framework for efficient VLLMs. InfoCarve consists of three stages. First, we adopt Dynamic Temporal Segmentation (DySeg)~\cite{shen2026fastvid} to partition sampled frames into temporally coherent segments, where spatio-temporal token compression is performed independently. Second,  existing FastV-style methods do not explicitly distinguish static and dynamic tokens. To address this issue, we propose a \textbf{Temporal Fingerprint Difference (TFD)} module to identify dynamically informative regions within each segment. Third, considering that different segments contain varying information density, we introduce an \textbf{Information-Density-Aware Budget Allocation (IDAB)} strategy to adaptively allocate token budgets across segments. Based on the proposed TFD and IDAB modules, InfoCarve progressively purges redundant video tokens while preserving informative spatio-temporal content. The retained video tokens are then combined with query tokens and fed into the LLM for response generation.

\subsection{Temporal Fingerprint Difference}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{latex/figures/MADD_editable_diagram.pdf}
\caption{Illustration of the proposed Temporal Fingerprint Difference (TFD). For each spatial position, we construct an intra-segment temporal similarity matrix and compute its frame-wise differences to estimate temporal dynamics. Smaller TFD values indicate higher temporal consistency and thus greater redundancy.}
    \label{fig:madd}
\end{figure}

Existing methods~\cite{shen2026fastvid} estimate temporal redundancy mainly through local similarities between adjacent frames. However, such short-range measurements are sensitive to frame-level noise and often fail to reliably distinguish temporally static tokens from dynamically informative ones. We argue that truly redundant tokens should exhibit globally consistent temporal patterns within a segment, rather than only local frame-to-frame similarity. 

To this end, we propose a \textbf{Temporal Fingerprint Difference (TFD)} module, which models segment-level temporal consistency for robust redundancy estimation, as illustrated in Fig.~\ref{fig:madd}. Given the video features $\mathbf{H}\in\mathbb{R}^{T\times N\times D}$, we first partition the video into temporally coherent segments using DySeg. For the $k$-th segment $\mathcal{V}_k$, let $\mathbf{H}^{(k)}_{s,p}\in\mathbb{R}^{D}$ denote the token at spatial position $p$ in frame $s$.

For each spatial position $p$, we first normalize token features across all frames,We then construct a temporal similarity fingerprint matrix:
\begin{equation}
\small
\mathbf{F}^{(k)}_p[s,s']
=
\mathbf{Cos}
\left(\frac{\mathbf{H}^{(k)}_{s,p}}{\|\mathbf{H}^{(k)}_{s,p}\|_2}, \frac{\mathbf{H}^{(k)}_{s',p}}{\|\mathbf{H}^{(k)}_{s',p}\|_2} 
\right),
\end{equation}
where \mathbf{Cos} dontes the cosine similarity function and
$\mathbf{F}^{(k)}_p\in\mathbb{R}^{S_k\times S_k}$ characterizes the pairwise temporal similarity structure of spatial position $p$ throughout the entire segment. Intuitively, temporally static regions (e.g., background or repeated semantics) tend to maintain stable similarity structures across time, while dynamic regions exhibit larger temporal variations. Based on this observation, we measure temporal dynamics by computing the first-order difference of the fingerprint matrix along the temporal dimension:

\begin{equation}
\vspace{-3mm}
\resizebox{0.9\linewidth}{!}{$
\mathrm{TFD}^{(k)}(p)
=
\frac{
\sum_{s=1}^{S_k-1}
\sum_{s'=1}^{S_k}
\left|
\mathbf{F}^{(k)}_p[s+1,s']
-
\mathbf{F}^{(k)}_p[s,s']
\right|} {(S_k-1)S_k}
$}
\end{equation}
A smaller TFD value indicates stronger temporal consistency and therefore a higher likelihood of redundancy. Accordingly, for each segment, we select the spatial positions with the smallest TFD scores as static candidates:
\begin{equation}
\mathcal{S}^{(k)}= \operatorname{Top}_{\lfloor \rho N \rfloor}
\left(-\mathrm{TFD}^{(k)}(p) \right),
\end{equation}
where $\rho$ controls the proportion of static candidates.

Instead of directly removing these tokens, we use the static candidate set as a redundancy prior for subsequent compression. Specifically, static positions receive lower preservation priority during token selection, reducing repeated retention of temporally redundant content while preserving important dynamic information.

\subsection{Information-Density-Aware Budget Allocation}
\label{sec:method:budget}

Existing methods such as FastV~\cite{shen2026fastvid} allocate token budgets to temporal segments mainly according to segment length. However, video information is often unevenly distributed across time. For example, long static segments may contain substantial temporal redundancy, while short action-intensive segments often carry richer semantic information and therefore require more visual tokens for accurate understanding. Motivated by this observation, we propose an \textbf{Information-Density-Aware Budget Allocation (IDAB)} strategy to dynamically allocate token budgets based on the estimated information content of each segment.

\paragraph{Segment Uniqueness.} Given $K$ temporal segments generated by DySeg, we first compute the segment-level feature representation for the $k$-th segment $\mathcal{V}_k$:
\begin{equation}
\bar{\mathbf{x}}_k
=\frac{1}{|\mathcal{V}_k|N}\sum_{s=1}^{|\mathcal{V}_k|}
\sum_{p=1}^{N}\mathbf{H}^{(k)}_{s,p},
\end{equation}
where $|\mathcal{V}_k|$ denotes the number of frames in the segment and $N$ is the number of spatial tokens per frame. We further compute the global video representation by aggregating all segment features:
\begin{equation}
\bar{\mathbf{x}}_{\mathrm{glob}}
=
\frac{
\sum_{k=1}^{K}
|\mathcal{V}_k|
\bar{\mathbf{x}}_k
}
{
\sum_{k=1}^{K}
|\mathcal{V}_k|
}.
\end{equation}

To measure how much unique information a segment contributes to the entire video, we define the \textbf{segment uniqueness} score as the cosine distance between the segment representation and the global video representation:
\begin{equation}
u_k = 1-\mathbf{Cos}(\bar{\mathbf{x}}_k, \bar{\mathbf{x}}_{\mathrm{glob}} ).
\end{equation}
A larger uniqueness score indicates that the segment deviates more from the dominant global semantics and is therefore more likely to contain informative or distinctive visual content. 

 

\paragraph{Information Density.}

While segment uniqueness measures semantic distinctiveness at the video level, it does not reflect the internal complexity of visual representations within a segment. We further observe that low-density segments usually exhibit highly concentrated feature distributions, where most token energy lies in only a few principal directions. In contrast, information-rich segments tend to have more dispersed feature spectra, indicating more complex visual semantics. Motivated by this observation, we estimate segment information density using spectral entropy.

For the $k$-th segment, we first flatten all visual tokens into a feature matrix:
$\mathbf{X}_k \in \mathbb{R}^{S_kN \times D}$, where $S_k$ denotes the number of frames and $N$ is the number of spatial tokens per frame. We then compute the singular values $\{\sigma_j\}_{j=1}^{R}$ of $\mathbf{X}_k$, where
$R=\min(S_kN,D).$ The normalized spectral energy distribution is defined as:
\begin{equation}
\pi_j
=
\frac{\sigma_j^2}
{\sum_{\ell=1}^{R}\sigma_\ell^2}.
\end{equation}
Based on this distribution, we compute the normalized spectral entropy as the information-density score:
\begin{equation}
e_k
=
\frac{
-\sum_{j=1}^{R}
\pi_j \log \pi_j
}{
\log R
}.
\end{equation}
A smaller $e_k$ indicates that the feature energy is concentrated in a few dominant directions, suggesting relatively simple and redundant visual content. In contrast, larger entropy values imply a more diverse feature spectrum and therefore richer semantic information.


\paragraph{Information-Density-Aware Budget Allocation.} To jointly model semantic uniqueness and representation complexity, we first apply z-score normalization to both metrics across all segments and then fuse them:
\begin{equation}
m_k = \alpha z(u_k) + \beta z(e_k),
\end{equation}
where $\alpha$ and $\beta$ balance the contributions of the two factors.
Finally, we convert the fused score into a budget allocation weight:
\begin{equation}
w_k =\sigma(\tau_{\mathrm{bud}} m_k)\cdot S_k,
\end{equation}
where $\tau_{\mathrm{bud}}$ controls the sharpness of budget redistribution. The final token budget for the $k$-th segment is computed as:
\begin{equation}
B_k = \max \left( 1,\operatorname{round}
\left( \frac{FT_c w_k} {\sum_{j=1}^{K} w_j} \right) \right),
\end{equation}
where $FT_c$ denotes the total available context-token budget.
In this way, IDAB adaptively allocates more tokens to semantically informative and structurally complex segments while suppressing redundant low-density regions.
 


\subsection{Spatio-Temporal Compression}
\label{sec:method:compression}

After obtaining the static candidate set $\mathcal{S}^{(k)}$ from TFD and the adaptive token budget $B_k$ from IDAB, we perform spatio-temporal token compression within each segment. Following FastVID~\cite{shen2026fastvid}, our framework consists of two complementary components: Attention-based Token Selection (ATS) for preserving salient fine-grained details, and Density-based Token Merging (DTM) for maintaining segment-level contextual information. Different from previous methods, both modules are guided by the temporal redundancy prior estimated by TFD, which suppresses repeated preservation of static content across frames.

\paragraph{Attention-based Token Selection.}

ATS aims to preserve visually salient tokens within each frame. Following prior work, we use the attention from the [CLS] token to patch tokens as a saliency estimate.   A straightforward frame-wise top-$k$ selection strategy often repeatedly preserves the same static background regions due to their consistently high attention responses. Although these regions may contain visually meaningful information, repeatedly allocating tokens to near-duplicate static content leads to inefficient token utilization.

%Since many Video-LLMs employ SigLIP as the visual encoder while discarding its original classification head, the corresponding [CLS] attention is unavailable during inference. Following FastVID, we re-attach the pretrained SigLIP head to obtain lightweight saliency estimation without modifying the original Video-LLM pipeline.


To alleviate this issue, we introduce a redundancy-aware soft suppression mechanism guided by the static candidate set $\mathcal{S}^{(k)}$. For frame $f$, let $\mathbf{A}_f\in\mathbb{R}^{N}$ denote the flattened [CLS]-to-patch attention scores. We further maintain a historical static set $\mathcal{P}^{(k)}_{f-1}$, which records the static positions that have already been selected in previous frames of segment $\mathcal{V}_k$. Based on this prior, the attention score for position $p$ is computed as: 
\begin{equation}
\resizebox{0.9\linewidth}{!}{$
\tilde{\mathbf{A}}_{f,p}=\bar{\mathbf{A}}_{f,p}
-\lambda \cdot \operatorname{std}(\bar{\mathbf{A}}_f)
\cdot \mathbb{1}
\left[
p\in\mathcal{S}^{(k)}
\land
p\in\mathcal{P}^{(k)}_{f-1}
\right],
}
\end{equation}
where $\lambda$ controls the suppression strength and $\mathbb{1}[\cdot]$ denotes the indicator function, which equals $1$ when the condition is satisfied and $0$ otherwise. Finally, ATS preserves the top-$T_s$ tokens according to the adjusted attention scores:
\begin{equation}
\mathcal{T}^{\mathrm{ATS}}_f
=
\operatorname{Top}_{T_s}
(
\tilde{\mathbf{A}}_f
).
\end{equation}
Unlike hard removal, this soft suppression still allows highly informative static tokens to survive when necessary, while encouraging more token budget to be allocated to newly emerging dynamic regions.

\paragraph{Hard-masked Density-based Token Merging.}

While ATS preserves salient local details, DTM is responsible for maintaining global contextual information within each segment. We first sample anchor frames at a fixed interval $p$. For the $k$-th segment, the number of anchor frames is:
\begin{equation}
n_a^{(k)} = \left\lceil \frac{S_k}{p}\right\rceil.
\end{equation}

Given the segment budget $B_k$, each anchor frame receives:
\begin{equation}
T_{c,a}^{(k)}
=
\left\lfloor
\frac{B_k}{n_a^{(k)}}
\right\rfloor
\end{equation}
context anchor tokens. Within each anchor frame, DTM selects representative tokens using density-peak clustering. For token $v_i$, its local density is computed as:
\begin{equation}
\rho_i
=
\exp
\left(
-
\frac{1}{K_{\mathrm{nn}}}
\sum_{v_j\in\mathrm{kNN}(v_i)}
d(v_i,v_j)^2
\right),
\end{equation}
and its distance to higher-density tokens is defined as:
\begin{equation}
\delta_i=
\begin{cases}
\min_{j:\rho_j>\rho_i}
d(v_i,v_j),
&
\exists j,\rho_j>\rho_i,
\\
\max_j d(v_i,v_j),
&
\text{otherwise}.
\end{cases}
\end{equation}
The final density-peak score is given by:
\begin{equation}
s_i=\rho_i\delta_i.
\end{equation}
However, without additional constraints, multiple anchor frames may repeatedly select the same static regions as cluster centers, leading to redundant context preservation. To improve spatial diversity, we introduce a redundancy-aware hard mask guided by TFD. Let $\mathcal{Q}^{(k)}_{a-1}$ denote the set of static positions already selected by previous anchor frames within segment $\mathcal{V}_k$. For the current anchor frame, if position $p$ belongs to $\mathcal{Q}^{(k)}_{a-1}$, its density score is directly suppressed:
\begin{equation}
s_{a,p}
\leftarrow
-\infty,
\quad
p\in\mathcal{Q}^{(k)}_{a-1}.
\end{equation}

The top-$T_{c,a}^{(k)}$ remaining tokens are then selected as context anchors. Compared with the soft suppression used in ATS, the hard mask in DTM explicitly prevents repeatedly selecting identical static centers across anchor frames, thereby improving contextual diversity and coverage.

\paragraph{Anchor-centric Aggregation.}

After anchor selection, each unreserved token is assigned to its nearest anchor center and merged into the corresponding anchor representation. For anchor token $a$ with assigned token set $\{b_1,\dots,b_n\}$, the updated representation is:
\begin{equation}
a^\star
=
\mu a
+
(1-\mu)
\frac{1}{n}
\sum_{j=1}^{n}b_j,
\end{equation}
where $\mu$ balances the original anchor feature and aggregated neighboring information. 
Finally, the salient tokens preserved by ATS and the contextual anchors generated by DTM are concatenated in temporal order to form the compressed video-token sequence, which is then fed into the LLM together with text tokens.

 

}

==> latex/section/related.tex <==
\subsection{Video Large Language Models}

The deep integration of large language models (LLMs) and vision transformers (ViTs) has given rise to vision-language models (VLMs), which have demonstrated strong capabilities in video understanding and question answering.
Early methods typically build upon image-based multimodal large language models by extracting video features with video encoders, such as VideoChat~\cite{li2025videochat} and VideoLLaMA~\cite{cheng2024videollama}, and further training the models on video instruction data.
Subsequently, models such as LLaVA-NeXT~\cite{liu2024llavanext}, LLaVA-OneVision~\cite{li2024llava-ov}, LLaVA-Video~\cite{zhang2024llava-video}, Qwen-VL~\cite{bai2025qwen3}, and InternVL-Video~\cite{wang2025internvl3} have further enhanced unified modeling across images, videos, and text.
Although these works reduce the number of visual tokens through operations such as pooling or pixel reshaping, the visual tokens passed to the downstream LLM can still reach the order of thousands, leading to substantial computational overhead.
Although recent works such as VILA~\cite{lin2024vila} and NVILA~\cite{liu2025nvila} aim to optimize token usage, they typically require model fine-tuning, which demands considerable computational resources.
Therefore, developing an efficient training-free token compression method is of critical importance.

\subsection{Visual Token Compression}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.98\textwidth]{figures/pipeline4.pdf}
    \caption{Overview of the proposed InfoMerge framework.}
    \label{fig:method}
\end{figure*}


Token compression is an effective way to reduce token redundancy in ViTs and LLMs.
According to where compression is performed, existing methods can be roughly categorized into compression outside the LLM, compression inside the LLM, and hybrid compression methods that combine both.
According to the type of redundancy being handled, these methods can also be divided into spatial redundancy compression, temporal redundancy compression, and joint spatio-temporal compression.
Spatial compression methods aim to reduce redundancy within each frame.ToMe~\cite{bolya2022tome} reduces the number of tokens in ViTs by merging similar tokens.VisionZip~\cite{yang2025visionzip} use attention scores from the visual encoder to estimate token importance, preferentially preserving salient regions.
FastV~\cite{chen2024image} prune visual tokens inside the LLM according to shallow-layer attention.
These methods mainly focus on spatial saliency, and are less effective at handling background regions and static areas that repeatedly appear across video frames.
In addition, pruning inside the LLM inevitably introduces a fixed early-layer overhead.

Temporal compression focuses on redundant information across frames.
DyCoke~\cite{tao2025dycoke}, TempMe~\cite{shen2025tempme}, and PruneVID~\cite{huang2025prunevid} reduce temporal redundancy by identifying and merging similar tokens across frames.
FastVID~\cite{shen2026fastvid} uses DySeg to perform dynamic temporal segmentation, followed by token pruning and merging within each segment.
But many methods still rely on local similarities between adjacent frames.

Spatio-temporal compression can be further divided into staged spatio-temporal compression and unified spatio-temporal compression.
FastVID~\cite{shen2026fastvid} combines dynamic segmentation with spatio-temporal merging.
HoliTom~\cite{shao2025holitom} starts from global redundancy awareness and uses dynamic programming for temporal organization and token merging.
Recent work also formulates compression as a unified spatio-temporal token allocation problem.
USTC~\cite{du2026unified} introduces a global retention pool that jointly considers token contribution and redundancy.

How to allocate a limited token budget across different video segments is also crucial.
Static budget allocation methods, such as FastVID~\cite{shen2026fastvid}, allocate the context-token budget according to segment length after temporal segmentation.
However, such methods are difficult to adapt to the non-uniform information density in real-world videos.
In contrast, dynamic budget allocation methods adjust token retention based on the input content or model behavior.DyCoke~\cite{tao2025dycoke} dynamically compresses visual tokens by exploiting attention variations across different layers inside the LLM, while HoliTom~\cite{shao2025holitom} adjusts temporal token organization from the perspective of global redundancy.
Despite the progress of these methods, existing spatio-temporal compression approaches still have two main limitations.
First, many methods~\cite{tao2025dycoke,shao2025holitom} still use local similarity as the criterion for temporal redundancy, relying on the cosine similarity between tokens at the same spatial position in adjacent frames.
The underlying assumption is that tokens with high similarity at the same spatial position in adjacent frames are more likely to represent static background or repeated semantics, and therefore can be compressed.
However, when a video contains slight camera motion or illumination changes, token representations at the same spatial position may be affected by non-semantic perturbations, making redundancy estimation based on adjacent-frame cosine similarity unstable.
Second, high-attention tokens are not always equivalent to high semantic contribution, and highly similar tokens are not necessarily safe to remove.
Especially under strict compression ratios, a compression method needs not only to remove low-contribution tokens, but also to prevent visual representations from collapsing into an overly low-dimensional semantic subspace. 


==> latex/table/3bench.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.95}
\caption{\textbf{Comparison of State-of-The-Art Methods on LLaVA-OneVision-7B.}
The A\%/B\% retention ratio indicates that A\% of the LLM input tokens are retained, and subsequently compressed to B\% during the LLM forward pass.
FLOPs are measured for the Qwen2-7B backbone prefill at 32 frames $\times$ 196 tokens/frame $+\,$50 text tokens (cross-checked with \texttt{calflops}).
\textbf{Best} results are in bold, \underline{second best} underlined.}
\label{tab:sota_ov7b}

\resizebox{\textwidth}{!}{%
\begin{tabular}{l c c c c c c c c c c c c}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{\shortstack{FLOPs\\(T)\,$\downarrow$}} & \multirow{2}{*}{\shortstack{FLOPs\\Ratio}} & \multirow{2}{*}{\shortstack{Retention\\Ratio}}
 & \multicolumn{4}{c}{VideoMME\,$\uparrow$} & \multirow{2}{*}{MVBench\,$\uparrow$} & \multirow{2}{*}{MLVU\,$\uparrow$} & \multirow{2}{*}{\shortstack{Long\\VideoBench\,$\uparrow$}} & \multicolumn{2}{c}{Avg.\,$\uparrow$} \\
\cmidrule(lr){5-8} \cmidrule(lr){12-13}
 & & & & Short & Medium & Long & Overall & & & & Score & \% \\
\midrule
\rowcolor{gray!12}
LLaVA-OV-7B & 98.6 & 100.0\% & 100\%      & 70.2 & 56.8 & 48.8 & 58.6 & 58.3 & 65.2            & 56.4              & 59.63 & 100.0 \\
\midrule
FastV         & 11.5 & 11.7\% & 100\%/5\%  & 58.4          & \underline{52.9} & \textbf{46.1} & 52.5          & 51.2          & --                & --              & 51.85          & 87.0 \\
VisionZip     & 4.8  & 4.9\%  & 5\%        & --            & --               & --            & 48.2          & 45.2          & --                & --              & 46.70          & 78.3 \\
FastVID       & 4.8  & 4.9\%  & 5\%        & 63.3          & 51.7             & 45.5          & \underline{54.0} & \underline{53.0} & \underline{58.88} & \underline{51.4} & \underline{54.32} & \underline{91.1} \\
\textbf{Ours} & 4.8  & 4.9\%  & 5\%        & \textbf{65.2} & \textbf{53.0}    & \underline{45.7} & \textbf{54.7} & \textbf{54.5} & \textbf{59.48}    & \textbf{52.1}    & \textbf{55.17} & \textbf{92.5} \\
\midrule
FastV         & 15.4 & 15.6\% & 100\%/10\% & 65.8          & 54.7          & \underline{47.8} & 56.1          & 51.7          & 57.7              & 52.1              & 54.40          & 91.2 \\
VisionZip     & 9.0  & 9.2\%  & 10\%       & 59.4          & 52.9          & 45.4          & 52.8          & 51.7          & 59.7              & 48.3              & 53.13          & 89.1 \\
FastVID       & 9.0  & 9.2\%  & 10\%       & 67.2          & 55.7          & 47.6          & \underline{56.8} & \underline{55.9} & \textbf{62.19}    & \textbf{55.7}    & \underline{57.65} & \underline{96.7} \\
\textbf{Ours} & 9.0  & 9.2\%  & 10\%       & \textbf{68.9} & \textbf{55.9} & \textbf{48.2} & \textbf{57.7} & \textbf{56.7} & \underline{61.64} & \underline{55.2} & \textbf{57.79} & \textbf{96.9} \\
\midrule
FastV         & 19.4 & 19.7\% & 100\%/15\% & 68.4          & 54.9          & 48.1          & 57.1          & 52.2          & 59.8              & 54.9              & 56.00          & 93.9 \\
VisionZip     & 13.3 & 13.5\% & 15\%       & 63.0          & 54.4          & \textbf{49.1} & 55.5          & 54.3          & 60.0              & 53.9              & 55.93          & 93.8 \\
MMG-Vid(AAAI2026) & 13.3 & 13.5\% & 15\%   & --            & --            & --            & \underline{57.9} & 56.5          & 61.6              & 55.9              & 57.98          & 97.2 \\
FastVID       & 13.3 & 13.5\% & 15\%       & \underline{69.3} & \underline{56.4} & 47.6          & 57.8 & \underline{56.0} & 62.93             & \underline{56.2} & \underline{58.23} & \underline{97.7} \\
\textbf{Ours} & 13.3 & 13.5\% & 15\%       & \textbf{69.6} & \textbf{56.8} & \underline{48.1} & \textbf{58.2} & \textbf{57.7} & \textbf{63.02} & \textbf{56.4}    & \textbf{58.83} & \textbf{98.7} \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> latex/table/3bench_new.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.95}
\caption{\textbf{Comparison of SOTA Methods on LLaVA-OneVision-7B.}
The A\%/B\% retention ratio indicates that A\% of the LLM input tokens are retained, and subsequently compressed to B\% during the LLM forward pass. 
\textbf{Best} results are in bold, \underline{second best} underlined.}
\label{tab:sota_ov7b}

\resizebox{\textwidth}{!}{%
\begin{tabular}{l c c c c c c c c c c c c}
\toprule
\multirow{2}{*}{Method} 
& \multirow{2}{*}{\shortstack{FLOPs\\(T)\,$\downarrow$}} 
& \multirow{2}{*}{\shortstack{FLOPs\\Ratio}} 
& \multirow{2}{*}{\shortstack{Retention\\Ratio}}
& \multicolumn{4}{c}{VideoMME\,$\uparrow$} 
& \multirow{2}{*}{MVBench\,$\uparrow$} 
& \multirow{2}{*}{MLVU\,$\uparrow$} 
& \multirow{2}{*}{\shortstack{Long\\VideoBench\,$\uparrow$}} 
& \multicolumn{2}{c}{Avg.\,$\uparrow$} \\
\cmidrule(lr){5-8} \cmidrule(lr){12-13}
& & & & Short & Medium & Long & Overall & & & & Score & \% \\
\midrule
\rowcolor{gray!12}
LLaVA-OV-7B 
& 48.8 & 100.0\% & 100\% 
& 70.2 & 56.8 & 48.8 & 58.6 & 58.3 & 65.2 & 56.4 & 59.63 & 100.0 \\
\midrule
FastV         
& 9.4 & 19.2\% & 100\%/15\% 
& 68.4 & 54.9 & 48.1 & 57.1 & 52.2 & 59.8 & 54.9 & 56.00 & 93.9 \\
VisionZip     
& 6.3 & 12.9\% & 15\% 
& 63.0 & 54.4 & \textbf{49.1} & 55.5 & 54.3 & 60.0 & 53.9 & 55.93 & 93.8 \\
MMG-Vid       
& 6.3 & 12.9\% & 15\% 
& -- & -- & -- & \underline{57.9} & 56.5 & 61.6 & 55.9 & 57.98 & 97.2 \\
FastVID       
& 6.3 & 12.9\% & 15\% 
& \underline{69.3} & \underline{56.4} & 47.6 & 57.8 & \underline{56.0} & 62.9 & \underline{56.2} & \underline{58.23} & \underline{97.7} \\
\textbf{Ours} 
& 6.3 & 12.9\% & 15\% 
& \textbf{69.6} & \textbf{56.8} & \underline{48.1} & \textbf{58.2} & \textbf{57.7} & \textbf{63.1} & \textbf{56.4} & \textbf{58.83} & \textbf{98.7} \\
\midrule
FastV         
& 7.4 & 15.1\% & 100\%/10\% 
& 61.7 & 54.1 & 47.1 & 54.3
& 51.7 & 57.7 & 52.1 & 54.40 & 91.2 \\
VisionZip     
& 4.2 & 8.5\% & 10\% 
& 59.4 & 52.9 & 45.4 & 52.8 & 51.7 & 59.7 & 48.3 & 53.13 & 89.1 \\
FastVID       
& 4.2 & 8.5\% & 10\% 
& 67.2 & 55.7 & 47.6 & \underline{56.8} & \underline{55.9} & \textbf{62.1} & \textbf{55.7} & \underline{57.65} & \underline{96.7} \\
\textbf{Ours} 
& 4.2 & 8.5\% & 10\% 
& \textbf{68.9} & \textbf{55.9} & \textbf{48.2} & \textbf{57.7} & \textbf{56.6} & \underline{61.7} & \underline{55.2} & \textbf{57.79} & \textbf{96.9} \\
\midrule
FastV         
& 5.4 & 11.1\% & 100\%/5\% 
& 56.3 & \underline{51.7} & \textbf{44.1} & 50.7 
& 51.2 & -- & 47.9 & 51.85 & 87.0 \\
VisionZip     
& 2.1 & 4.2\% & 5\% 
& 60.3 & 52.1 & 46.3 & 52.9 & 45.2 & -- & 46.6 & 46.70 & 78.3 \\
FastVID       
& 2.1 & 4.2\% & 5\% 
& 63.3 & 51.7 & 45.5 & \underline{54.0} & \underline{53.0} & \underline{58.8} & \underline{51.4} & \underline{54.32} & \underline{91.1} \\
\textbf{Ours} 
& 2.1 & 4.2\% & 5\% 
& \textbf{65.2} & \textbf{53.0} & \underline{45.7} & \textbf{54.6} & \textbf{54.5} & \textbf{59.5} & \textbf{52.1} & \textbf{55.17} & \textbf{92.5} \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> latex/table/bench3.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.95}
\caption{\textbf{Comparison of SOTA Methods on LLaVA-OneVision-7B.}
The A\%/B\% retention ratio indicates that A\% of the LLM input tokens are retained, and subsequently compressed to B\% during the LLM forward pass. 
\textbf{Best} results are in bold, \underline{second best} underlined.}
\label{tab:sota_ov7b}

\resizebox{\textwidth}{!}{%
\begin{tabular}{l c c c c c c c c c c c}
\toprule
\multirow{2}{*}{Method} 
& \multirow{2}{*}{\shortstack{FLOPs\\(T)\,$\downarrow$}} 
& \multirow{2}{*}{\shortstack{FLOPs\\Ratio}} 
& \multirow{2}{*}{\shortstack{Retention\\Ratio}}
& \multicolumn{4}{c}{VideoMME\,$\uparrow$} 
& \multirow{2}{*}{MLVU\,$\uparrow$} 
& \multirow{2}{*}{\shortstack{Long\\VideoBench\,$\uparrow$}} 
& \multicolumn{2}{c}{Avg.\,$\uparrow$} \\
\cmidrule(lr){5-8} \cmidrule(lr){11-12}
& & & & Short & Medium & Long & Overall & & & Score & \% \\
\midrule
\rowcolor{gray!12}
LLaVA-OV-7B 
& 48.8 & 100.0\% & 100\% 
& 70.2 & 56.8 & 48.8 & 58.6 
& 65.2 & 56.4 & 59.63 
& 100.0 \\
\midrule
FastV         
& 9.4 & 19.2\% & 100\%/15\% 
& 65.6 & 55.1 & 46.9 & 55.9 
& 60.2 & 532 
& 56.00 & 93.9 \\
VisionZip     
& 6.3 & 12.9\% & 15\% 
& 63.0 & 54.4 & \textbf{49.1} & 55.5 
& 60.0 & 53.9 
& 55.93 & 93.8 \\
MMG-Vid       
& 6.3 & 12.9\% & 15\% 
& -- & -- & -- & \underline{57.9} & 61.6 & 55.9 & 57.98 & 97.2 \\
FastVID       
& 6.3 & 12.9\% & 15\% 
& \underline{69.3} & \underline{56.4} & 47.6 & 57.8 & 62.9 & \underline{56.2} & \underline{58.23} & \underline{97.7} \\
\textbf{Ours} 
& 6.3 & 12.9\% & 15\% 
& \textbf{69.6} & \textbf{56.8} & \underline{48.1} & \textbf{58.2} & \textbf{63.1} & \textbf{56.4} & \textbf{58.83} & \textbf{98.7} \\
\midrule
FastV         
& 7.4 & 15.1\% & 100\%/10\% 
& 61.7 & 54.1 & 47.1 & 54.3 
& 58.6 & 52.1 
& 54.40 & 91.2 \\
VisionZip     
& 4.2 & 8.5\% & 10\% 
& 59.4 & 52.9 & 45.4 & 52.8 & 59.7 & 48.3 & 53.13 & 89.1 \\
FastVID       
& 4.2 & 8.5\% & 10\% 
& 67.2 & 55.7 & 47.6 & \underline{56.8} & \textbf{62.1} & \textbf{55.7} & \underline{57.65} & \underline{96.7} \\
\textbf{Ours} 
& 4.2 & 8.5\% & 10\% 
& \textbf{68.9} & \textbf{55.9} & \textbf{48.2} & \textbf{57.7} & \underline{61.7} & \underline{55.2} & \textbf{57.79} & \textbf{96.9} \\
\midrule
FastV         
& 5.4 & 11.1\% & 100\%/5\% 
& 56.3 & \underline{51.7} & 44.1 & 50.7 
& 56.1 & 48.5 
& 51.85 & 87.0 \\
VisionZip     
& 2.1 & 4.2\% & 5\% 
& 60.3 & 52.1 & \textbf{46.3} & 52.9 & -- & 46.6 & 46.70 & 78.3 \\
FastVID       
& 2.1 & 4.2\% & 5\% 
& 63.3 & 51.7 & 45.5 & \underline{54.0} & \underline{58.8} & \underline{51.4} & \underline{54.32} & \underline{91.1} \\
\textbf{Ours} 
& 2.1 & 4.2\% & 5\% 
& \textbf{65.2} & \textbf{53.0} & \underline{45.7} & \textbf{54.6} & \textbf{59.5} & \textbf{52.1} & \textbf{55.17} & \textbf{92.5} \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> latex/table/chengfa.tex <==

% -----------------------------------------------------
% Table 4: MADD penalty sensitivity
% -----------------------------------------------------
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{\textbf{Effect of the TFD penalty weight \lambda} on VideoMME at $r=0.10$
(50-sample subset used for sweep efficiency).
$p=10^{9}$ corresponds to the original FastVID hard cut-off.
A moderate penalty ($p\!\geq\!8$) recovers most of the gain;
$p\in[10,15]$ saturates.}
\label{tab:abl_madd}
\begin{tabular}{l c c c c c c c c}
\toprule
$p$ & 1 & 2 & 5 & 8 & 10 & 12 & 15 & $10^{9}$ \\
\midrule
VideoMME-50 & 57.30 & 57.11 & 57.30 & 57.44 & \textbf{57.67} & \textbf{57.67} & \textbf{57.67} & 57.67 \\
\bottomrule
\end{tabular}
\end{table}


==> latex/table/compar1.tex <==
\iffasle

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{\textbf{Comparison of State-of-The-Art Methods on LLaVA-OneVision-7B.}
The A\%/B\% retention ratio indicates that A\% of the LLM input tokens are retained, and subsequently compressed to B\% during the LLM forward pass.
\textbf{Best} results are in bold, \underline{second best} underlined.}
\label{tab:sota_ov7b}
\begin{tabular}{l c c c c c c c c c c}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{\shortstack{FLOPs\\(T)\,$\downarrow$}} & \multirow{2}{*}{\shortstack{FLOPs\\Ratio}} & \multirow{2}{*}{\shortstack{Retention\\Ratio}}
 & \multicolumn{4}{c}{VideoMME\,$\uparrow$} & \multirow{2}{*}{MVBench\,$\uparrow$} & \multicolumn{2}{c}{Avg.\,$\uparrow$} \\
\cmidrule(lr){5-8} \cmidrule(lr){10-11}
 & & & & Short & Medium & Long & Overall & & Score & \% \\
\midrule
\rowcolor{gray!12}
LLaVA-OV-7B & 41.4 & 100\%   & 100\%      & 70.2 & 56.8 & 48.8 & 58.6 & 58.3 & 58.45 & 100.0 \\
\midrule
FastV         & 6.4 & 15.5\% & 100\%/5\%  & --            & --            & --            & 49.7          & 51.2          & 50.45          & 86.3 \\
VisionZip     & 2.2 & 5.4\%  & 5\%        & --            & --            & --            & 48.2          & 45.2          & 46.70          & 79.9 \\
FastVID       & 2.2 & 5.4\%  & 5\%        & 63.3            & 51.7            & 45.5            & \underline{54.0} & \underline{53.0} & \underline{53.50} & \underline{91.5} \\
\textbf{Ours} & 2.2 & 5.4\%  & 5\%        & \textbf{65.2} & \textbf{53.0} & \textbf{45.7} & \textbf{54.6} & \textbf{54.5} & \textbf{54.55} & \textbf{93.3} \\
\midrule
FastV         & 7.9 & 19.1\% & 100\%/10\% & --            & --            & --            & 52.7          & 51.7          & 52.20          & 89.3 \\
VisionZip     & 4.0 & 9.6\%  & 10\%       & --            & --            & --            & 53.4          & 51.7          & 52.55          & 89.9 \\
FastVID       & 4.0 & 9.6\%  & 10\%       & 67.2          & 55.7          & 47.6          & \underline{56.8} & \underline{55.9} & \underline{56.35} & \underline{96.4} \\
\textbf{Ours} & 4.0 & 9.6\%  & 10\%       & \textbf{68.9} & \textbf{55.9} & \textbf{48.2} & \textbf{57.7} & \textbf{56.6} & \textbf{57.15} & \textbf{97.8} \\
\midrule
FastV         & 9.4 & 22.7\% & 100\%/15\% & --            & --            & --            & 54.7          & 53.2          & 53.95          & 92.3 \\
VisionZip     & 5.8 & 14.0\% & 15\%       & --            & --            & --            & 56.1          & 54.3          & 55.21          & 94.5 \\
FastVID       & 5.8 & 14.0\% & 15\%       & \underline{69.3} & \underline{56.4} & \underline{47.6} & \underline{57.8} & \underline{56.0} & \underline{56.85} & \underline{97.3} \\
\textbf{Ours} & 5.8 & 14.0\% & 15\%       & \textbf{69.6} & \textbf{56.8} & \textbf{48.1} & \textbf{58.2} & \textbf{57.7} & \textbf{57.95} & \textbf{99.1} \\
\bottomrule
\end{tabular}
\end{table*}
\fi




\begin{table*}[t]
\centering
\caption{\textbf{Comparison of State-of-The-Art Methods on LLaVA-OneVision-7B.}
The A\%/B\% retention ratio indicates that A\% of the LLM input tokens are retained, and subsequently compressed to B\% during the LLM forward pass.
\textbf{Best} results are in bold, \underline{second best} underlined.}
\label{tab:token_reduction}
	\resizebox{0.97\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\toprule
\multirow{2}{*}{Method} & FLOPs & FLOPs & Retention & \multicolumn{4}{c}{VideoMME $\uparrow$} & \multirow{2}{*}{MVBench $\uparrow$} & \multicolumn{2}{c}{Avg. $\uparrow$} \\
\cmidrule(lr){5-8} \cmidrule(lr){10-11}
 & (T) $\downarrow$ & Ratio & Ratio & Short & Medium & Long & Overall & & Score & \% \\
\midrule
\rowcolor{gray!12} LLaVA-OV-7B & 41.4 & 100\% & 100\% & 70.2 & 56.8 & 48.8 & 58.6 & 58.3 & 58.45 & 100.0 \\
\midrule
FastV & 6.4 & 15.5\% & 100\%/5\% & -- & -- & -- & 49.7 & 51.2 & 50.45 & 86.3 \\
VisionZip & 2.2 & 5.4\% & 5\% & -- & -- & -- & 48.2 & 45.2 & 46.70 & 79.9 \\
FastVID & 2.2 & 5.4\% & 5\% & 63.3 & 51.7 & 45.5 & 54.0 & 53.0 & 53.50 & 91.5 \\
\textbf{Ours} & \textbf{2.2} & \textbf{5.4\%} & \textbf{5\%} & \textbf{65.2} & \textbf{53.0} & \textbf{45.7} & \textbf{54.6} & \textbf{54.5} & \textbf{54.55} & \textbf{93.3} \\
\midrule
FastV & 7.9 & 19.1\% & 100\%/10\% & -- & -- & -- & 52.7 & 51.7 & 52.20 & 89.3 \\
VisionZip & 4.0 & 9.6\% & 10\% & -- & -- & -- & 53.4 & 51.7 & 52.55 & 89.9 \\
FastVID & 4.0 & 9.6\% & 10\% & \underline{67.2} & \underline{55.7} & \underline{47.6} & \underline{56.8} & \underline{55.9} & \underline{56.35} & \underline{96.4} \\
\textbf{Ours} & \textbf{4.0} & \textbf{9.6\%} & \textbf{10\%} & \textbf{68.9} & \textbf{55.9} & \textbf{48.2} & \textbf{57.7} & \textbf{56.6} & \textbf{57.15} & \textbf{97.8} \\
\midrule
FastV & 9.4 & 22.7\% & 100\%/15\% & -- & -- & -- & 54.7 & 53.2 & 53.95 & 92.3 \\
VisionZip & 5.8 & 14.0\% & 15\% & -- & -- & -- & 56.1 & 54.3 & 55.21 & 94.5 \\
FastVID & 5.8 & 14.0\% & 15\% & \underline{69.3} & \underline{56.4} & \underline{47.6} & \underline{57.8} & \underline{56.0} & \underline{56.85} & \underline{97.3} \\
\textbf{Ours} & \textbf{5.8} & \textbf{14.0\%} & \textbf{15\%} & \textbf{69.6} & \textbf{56.8} & \textbf{48.1} & \textbf{58.2} & \textbf{57.7} & \textbf{57.95} & \textbf{99.1} \\
\bottomrule
\end{tabular}}
\end{table*}

==> latex/table/lantency.tex <==
\begin{table}[t]
\centering
\caption{Efficiency comparison following MMG-Vid Table 2. Prefill is time to first generated token; generate is time from first token to response end.}
\label{tab:table2-phase-latency}
\small
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{Prefill Time (ms)} & \textbf{Generate Time (ms)} & \textbf{Samples} \\
\midrule
LLaVA-OV & 744.2 (1.00x) & 1677.9 (1.00x) & 30 \\
Ours $r{=}5\%$ & 730.5 (1.02x) & 632.2 (2.65x) & 30 \\
Ours $r{=}7.5\%$ & 736.6 (1.01x) & 673.7 (2.49x) & 30 \\
\bottomrule
\end{tabular}
\end{table}


==> latex/table/llavavideo.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\caption{\textbf{VideoMME results on LLaVA-Video-7B-Qwen2.}
Original FastVID is compared with our dynamic allocation method at the same retention ratio.
\textbf{Best} results under each retention ratio are in bold.}
\label{tab:videomme_llavavideo_fastvid_ours}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l c c c c c c}
\toprule
Method & Retention & Short & Medium & Long & Overall & $\Delta$ Overall \\
\midrule
FastVID & 5\%  & 68.7 & \textbf{56.9} & \textbf{49.2} & \textbf{58.3} & -- \\
\textbf{Ours} & 5\%  & \textbf{68.9} & 56.3 & 46.6 & 57.3 & -1.0 \\
\midrule
FastVID & 10\% & 72.0 & 58.1 & 50.4 & 60.2 & -- \\
\textbf{Ours} & 10\% & \textbf{72.6} & \textbf{59.1} & \textbf{51.0} & \textbf{60.9} & +0.7 \\
\midrule
FastVID & 15\% & \textbf{73.8} & 61.0 & 51.7 & 62.1 & -- \\
\textbf{Ours} & 15\% & 73.4 & \textbf{63.0} & \textbf{51.9} & \textbf{62.8} & +0.6 \\
\bottomrule
\end{tabular}}
\end{table}


==> latex/table/llavavideo2.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4.5pt}
\caption{\textbf{Comparison of state-of-the-art methods on LLaVA-Video-7B-Qwen2.}
We report results on MVBench and VideoMME.
FLOPs are measured under the default 64-frame setting.
\textbf{Best} results under each retention ratio are in bold.
``\%'' denotes the percentage of the Vanilla average score retained.
Empty entries indicate results that are not yet available.}
\label{tab:llava_video_sota}
\resizebox{\textwidth}{!}{
\begin{tabular}{l c c c c c c c c c c}
\toprule
\multirow{2}{*}{Method} 
& \multirow{2}{*}{\shortstack{Retention\\Ratio $R$}} 
& \multirow{2}{*}{\shortstack{FLOPs\\(T)$\downarrow$}} 
& \multirow{2}{*}{\shortstack{FLOPs\\Ratio}} 
& \multirow{2}{*}{MVBench} 
& \multicolumn{4}{c}{VideoMME} 
& \multirow{2}{*}{\shortstack{Avg.\\Score}} 
& \multirow{2}{*}{\%} \\
\cmidrule(lr){6-9}
& & & & & Overall & Short & Medium & Long & & \\
\midrule
\rowcolor{gray!12}
LLaVA-Video-7B
& 100\% & 94.1 & 100\% & 60.4 & 64.1 & 77.0 & 62.3 & 53.1  & -- & 100 \\

\midrule
FastV~\cite{chen2024image} 
& 10\% & 13.1 & -- & -- & -- & -- & -- & -- & -- & -- \\
VisionZip~\cite{yang2025visionzip} 
& 10\% & 6.9 & -- & -- & -- & -- & -- & -- & -- & -- \\
MMG-Vid 
& 10\% & 6.9 & -- & 54.9 & 59.4 & -- & -- & -- & -- & -- \\
FastVID 
& 10\% & 6.9 & -- & 58.5 & 60.2 & 72.0 & 58.1 & 50.4 & -- & -- \\
\textbf{Ours} 
& 10\% & 6.9 & -- & \textbf{60.0} & \textbf{60.9} & \textbf{72.6} & \textbf{59.1} & \textbf{51.0} & \textbf{60.5} & -- \\

\midrule
FastV~\cite{chen2024image} 
& 15\% & 16.9 & -- & -- & -- & -- & -- & -- & -- & -- \\
VisionZip~\cite{yang2025visionzip} 
& 15\% & 11.0 & -- & -- & -- & -- & -- & -- & -- & -- \\
MMG-Vid 
& 15\% & 11.0 & -- & 56.1 & 61.1 & -- & -- & -- & -- & -- \\
FastVID 
& 15\% & 11.0 & -- & \textbf{60.1} & 62.1 & \textbf{73.8} & 61.0 & 51.7 & -- & -- \\
\textbf{Ours} 
& 15\% & 11.5 & -- & \underline{59.9} & \textbf{62.8} & 73.4 & \textbf{63.0} & \textbf{51.9} & \textbf{61.4} & -- \\

% \midrule
% FastV~\cite{chen2024image} 
% & 5\% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% VisionZip~\cite{yang2025visionzip} 
% & 5\% & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% FastVID 
% & 5\% & -- & -- & 57.8 & \textbf{58.3} & 68.7 & \textbf{56.9} & \textbf{49.2} & \textbf{58.1} & -- \\
% \textbf{Ours} 
% & 5\% & -- & -- & \textbf{58.1} & 57.3 & \textbf{68.9} & 56.3 & 46.6 & 57.7 & -- \\

\bottomrule
\end{tabular}
}
\end{table*}

==> latex/table/llavavideo3.tex <==
% \begin{table*}[t]
% \centering
% \small
% \setlength{\tabcolsep}{4.5pt}
% \caption{\textbf{Comparison of SOTA methods on LLaVA-Video-7B-Qwen2.}
% We report results on MVBench and VideoMME.
% FLOPs are measured under the default 64-frame setting. 
% ``\%'' denotes the percentage of the Vanilla average score retained.}
% \label{tab:llava_video_sota}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l c c c c c c c c c c}
% \toprule
% \multirow{2}{*}{Method} 
% & \multirow{2}{*}{\shortstack{Retention\\Ratio $R$}} 
% & \multirow{2}{*}{\shortstack{FLOPs\\(T)$\downarrow$}} 
% & \multirow{2}{*}{\shortstack{FLOPs\\Ratio}} 
% & \multirow{2}{*}{MVBench} 
% & \multicolumn{4}{c}{VideoMME} 
% & \multirow{2}{*}{\shortstack{Avg.\\Score}} 
% & \multirow{2}{*}{\%} \\
% \cmidrule(lr){6-9}
% & & & & & Overall & Short & Medium & Long & & \\
% \midrule
% \rowcolor{gray!12}
% LLaVA-Video-7B
% & 100\% & 94.1 & 100.0\% 
% & 60.4 & 64.1 & 77.0 & 62.3 & 53.1 
% & 62.3 & 100.0 \\

% \midrule
% FastV~\cite{chen2024image}%(ECCV 2024)
% & 15\% & 16.9 & 18.0\%
% & 50.8 
% & 54.0 & 60.9 & 54.4 & 46.7 
% & 50.5 & 81.0 \\

% VisionZip~\cite{yang2025visionzip} %(CVPR 2025)
% & 15\% & 11.0 & 11.7\%
% & 55.2 
% & 60.3 & 70.3 & 58.8 & \underline{51.7}
% & 57.8 & 92.8 \\

% MMG-Vid~\cite{ma2026mmg} %(AAAI 2026)
% & 15\% & 11.0 & 11.7\%
% & 56.1 
% & 61.1 & 72.3 & 60.1 & 50.8
% & 58.6 & 94.1 \\

% FastVID~\cite{shen2026fastvid} %(NeurIPS 2025)
% & 15\% & 11.0 & 11.7\%
% & \textbf{60.5}
% & \underline{62.1} & \textbf{73.8} & \underline{61.0} & \underline{51.7}
% & \underline{61.1} & \underline{98.2} \\

% \textbf{Ours} 
% & 15\% & 11.0 & 11.7\%
% & \underline{59.9} 
% & \textbf{62.8} & \underline{73.4} & \textbf{63.0} & \textbf{51.9}
% & \textbf{61.4} & \textbf{98.6} \\

% \midrule
% FastV~\cite{chen2024image}%(ECCV 2024)
% & 10\% & 13.1 & 13.9\%
% & 43.2 
% & 49.6 & 67.6 & 57.5 & 48.6
% & 46.4 & 74.5 \\

% VisionZip~\cite{yang2025visionzip} %(CVPR 2025)
% & 10\% & 6.9 & 7.3\%
% & 53.8 & 58.7 & 67.4 & 57.7 & \textbf{51.1}
% & 56.3 & 90.4 \\

% MMG-Vid~\cite{ma2026mmg} %(AAAI 2026)
% & 10\% & 6.9 & 7.3\%
% & 54.9 & 59.4 & 71.0 & 57.9 & 49.2
% & 57.2 & 91.8 \\

% FastVID~\cite{shen2026fastvid} %(NeurIPS 2025)
% & 10\% & 6.9 & 7.3\%
% & \underline{58.5} & \underline{60.2} & \underline{72.0} & \underline{58.1} & 50.4
% & \underline{59.4} & \underline{95.3} \\

% \textbf{Ours} 
% & 10\% & 6.9 & 7.3\%
% & \textbf{60.0} & \textbf{60.9} & \textbf{72.6} & \textbf{59.1} & \underline{51.0}
% & \textbf{60.5} & \textbf{97.1} \\

% \bottomrule
% \end{tabular}
% }
% \end{table*}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4.5pt}
\caption{\textbf{Cross-backbone Method Comparison on LLaVA-Video-7B-Qwen2.}
We report results on MVBench and VideoMME.
FLOPs are measured under the default 64-frame setting.}
\label{tab:llava_video_sota}
\resizebox{\textwidth}{!}{
\begin{tabular}{l c c c c c c c c c c}
\toprule
\multirow{2}{*}{Method} 
& \multirow{2}{*}{\shortstack{Retention\\Ratio $R$}} 
& \multirow{2}{*}{\shortstack{FLOPs\\(T)$\downarrow$}} 
& \multirow{2}{*}{\shortstack{FLOPs\\Ratio}} 
& \multirow{2}{*}{MVBench} 
& \multicolumn{4}{c}{VideoMME} 
& \multirow{2}{*}{\shortstack{Avg.\\Score}} 
& \multirow{2}{*}{\%} \\
\cmidrule(lr){6-9}
& & & & & Overall & Short & Medium & Long & & \\
\midrule
\rowcolor{gray!12}
LLaVA-Video-7B
& 100\% & 94.1 & 100.0\% 
& 60.4 & 64.1 & 77.0 & 62.3 & 53.1 
& 62.3 & 100.0 \\

\midrule
FastV~\cite{chen2024image}
& 15\% & 16.9 & 18.0\%
& 50.8 
& 54.0 & 60.9 & 54.4 & 46.7 
& 52.4 & 84.2 \\

VisionZip~\cite{yang2025visionzip}
& 15\% & 11.0 & 11.7\%
& 55.2 
& 60.3 & 70.3 & 58.8 & \underline{51.7}
& 57.8 & 92.8 \\

MMG-Vid~\cite{ma2026mmg}
& 15\% & 11.0 & 11.7\%
& 56.1 
& 61.1 & 72.3 & 60.1 & 50.8
& 58.6 & 94.1 \\

FastVID~\cite{shen2026fastvid}
& 15\% & 11.0 & 11.7\%
& \textbf{60.5}
& \underline{62.1} & \textbf{73.8} & \underline{61.0} & \underline{51.7}
& \underline{61.3} & \underline{98.5} \\

\textbf{Ours} 
& 15\% & 11.0 & 11.7\%
& \underline{59.9} 
& \textbf{62.8} & \underline{73.4} & \textbf{63.0} & \textbf{51.9}
& \textbf{61.4} & \textbf{98.6} \\

\midrule
FastV~\cite{chen2024image}
& 10\% & 13.1 & 13.9\%
& 43.2 
& 49.6 & 54.0 & 50.3 & 44.6
& 46.4 & 74.5 \\

VisionZip~\cite{yang2025visionzip}
& 10\% & 6.9 & 7.3\%
& 53.8 & 58.7 & 67.4 & 57.7 & \textbf{51.1}
& 56.3 & 90.4 \\

MMG-Vid~\cite{ma2026mmg}
& 10\% & 6.9 & 7.3\%
& 54.9 & 59.4 & 71.0 & 57.9 & 49.2
& 57.2 & 91.8 \\

FastVID~\cite{shen2026fastvid}
& 10\% & 6.9 & 7.3\%
& \underline{58.5} & \underline{60.2} & \underline{72.0} & \underline{58.1} & 50.4
& \underline{59.4} & \underline{95.3} \\

\textbf{Ours} 
& 10\% & 6.9 & 7.3\%
& \textbf{60.0} & \textbf{60.9} & \textbf{72.6} & \textbf{59.1} & \underline{51.0}
& \textbf{60.5} & \textbf{97.1} \\

\bottomrule
\end{tabular}
}
\end{table*}

==> latex/table/multibench.tex <==
% -----------------------------------------------------
% Table 7: Retention ratio sweep across benchmarks
% -----------------------------------------------------
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\caption{\textbf{Retention-ratio sweep across benchmarks.}
``FastVID'' is the original FastVID (paper default), ``Ours'' is the
chosen $(\alpha,\beta,\gamma)=(0.9,0.0,0.1)$ configuration with
$\text{min}=0.1$, $p=12$, $\tau=1.2$, static-topk $=0.09$.
Numbers are overall scores (VideoMME perception score / MVBench average accuracy / EgoSchema subset accuracy).
\textbf{Best} per column in bold.}
\label{tab:abl_retention}
\begin{tabular}{l l c c c c c c}
\toprule
Benchmark & Method & $r=0.05$ & $r=0.075$ & $r=0.10$ & $r=0.15$ & $r=0.20$ & $r=1.0$ \\
\midrule
\multirow{2}{*}{VideoMME}
 & FastVID (orig) & 54.00$^{\dagger}$ & --     & 56.80 & 57.78 & 57.11 & \multirow{2}{*}{58.59} \\
 & Ours           & \textbf{54.55}    & 55.56  & \textbf{57.67} & \textbf{57.81} & \textbf{57.15} &  \\
\midrule
\multirow{2}{*}{MVBench}
 & FastVID (orig) & --                & --     & 57.13 & --    & --    & -- \\
 & Ours           & 54.48             & --     & 56.48 & \textbf{57.70} & \textbf{57.98} & -- \\
\midrule
\multirow{2}{*}{EgoSchema}
 & FastVID (orig) & 0.602             & --     & 0.586 & 0.598 & 0.616 & 0.622 \\
 & Ours           & \textbf{0.594}    & 0.586  & \textbf{0.594} & 0.596$^{\ddagger}$ & \textbf{0.616} & -- \\
\bottomrule
\end{tabular}
\vspace{2pt}\\
\footnotesize $^{\dagger}$ 50-sample subset only (full run not collected).
$^{\ddagger}$ $\tau=2.0$ variant used because $\tau=1.2$ failed; representative.
\end{table*}

==> latex/table/outMV.tex <==
% \begin{table*}[t]
% \centering
% \small
% \setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{0.95}
% \caption{\textbf{Comparison of SOTA Methods on LLaVA-OneVision-7B.}
% The A\%/B\% retention ratio indicates that A\% of the LLM input tokens are retained, and subsequently compressed to B\% during the LLM forward pass.
% \textbf{Best} results are in bold, \underline{second best} underlined.}
% \label{tab:sota_ov7b}

% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l c c c c c c c c c c c}
% \toprule
% \multirow{2}{*}{Method}
% & \multirow{2}{*}{\shortstack{FLOPs\\(T)\,$\downarrow$}}
% & \multirow{2}{*}{\shortstack{FLOPs\\Ratio}}
% & \multirow{2}{*}{\shortstack{Retention\\Ratio}}
% & \multicolumn{4}{c}{VideoMME\,$\uparrow$}
% & \multirow{2}{*}{MLVU\,$\uparrow$}
% & \multirow{2}{*}{\shortstack{Long\\VideoBench\,$\uparrow$}}
% & \multicolumn{2}{c}{Avg.\,$\uparrow$} \\
% \cmidrule(lr){5-8} \cmidrule(lr){11-12}
% & & & & Short & Medium & Long & Overall & & & Score & \% \\
% \midrule
% \rowcolor{gray!12}
% LLaVA-OV-7B
% & 48.8 & 100.0\% & 100\%
% & 70.2 & 56.8 & 48.8 & 58.6
% & 64.9 & 56.4 
% & 59.97 & 100.0 \\
% \midrule
% FastV
% & 9.4 & 19.2\% & 100\%/15\%
% & 65.6 & 55.1 & 46.9 & 55.9
% & 60.2 & 53.2 
% & 56.43 & 94.1 \\
% VisionZip
% & 6.3 & 12.9\% & 15\%
% & 67.4 & \textbf{57.6} & \textbf{48.1} & 57.7
% & 60.0 & 55.8 
% & 56.47 & 94.2 \\
% MMG-Vid
% & 6.3 & 12.9\% & 15\%
% & -- & -- & -- & \underline{57.9}
% & 61.6 & 55.9 
% & 58.47 & 97.5 \\
% FastVID
% & 6.3 & 12.9\% & 15\%
% & \underline{69.3} & \underline{56.4} & 47.6 & 57.8
% & \underline{62.9} & \underline{56.2}
% & \underline{58.97} & \underline{98.3} \\
% \textbf{Ours}
% & 6.3 & 12.9\% & 15\%
% & \textbf{69.6} & \textbf{56.8} & \textbf{48.1} & \textbf{58.2}
% & \textbf{63.1} & \textbf{56.4}
% & \textbf{59.23} & \textbf{98.8} \\
% \midrule
% FastV
% & 7.4 & 15.1\% & 100\%/10\%
% & 61.7 & 54.1 & 47.1 & 54.3
% & 58.6 & 52.1 
% & 55.00 & 91.7 \\
% VisionZip
% & 4.2 & 8.5\% & 10\%
% & 63.6 & \textbf{56.0} & \textbf{48.2} & 55.9
% & 59.7 & 54.5 
% & 54.63 & 91.1 \\
% FastVID
% & 4.2 & 8.5\% & 10\%
% & \underline{67.2} & 55.7 & \underline{47.6} & \underline{56.8}
% & \textbf{62.1} & \textbf{55.7}
% & \textbf{58.20} & \textbf{97.1} \\
% \textbf{Ours}
% & 4.2 & 8.5\% & 10\%
% & \textbf{68.9} & \underline{55.9} & \textbf{48.2} & \textbf{57.7}
% & \underline{61.7} & \underline{55.2}
% & \textbf{58.20} & \textbf{97.1} \\
% \midrule
% FastV
% & 5.4 & 11.1\% & 100\%/5\%
% & 56.3 & \underline{51.7} & \textbf{50.7} & 50.7
% & 56.1 & 48.5
% & 51.77 & 86.3 \\
% VisionZip
% & 2.1 & 4.2\% & 5\%
% & 59.8 & \underline{51.7} & \underline{45.9} & 52.4
% & 58.5 & 48.4 
% & -- & -- \\
% FastVID
% & 2.1 & 4.2\% & 5\%
% & \underline{63.3} & \underline{51.7} & 45.5 & \underline{54.0}
% & \underline{58.8} & \underline{51.4}
% & \underline{54.73} & \underline{91.3} \\
% \textbf{Ours}
% & 2.1 & 4.2\% & 5\%
% & \textbf{65.2} & \textbf{53.0} & 45.7 & \textbf{54.6}
% & \textbf{59.5} & \textbf{52.1}
% & \textbf{55.40} & \textbf{92.4} \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.95}
\caption{\textbf{Comparison of SOTA Methods on LLaVA-OneVision-7B.}
The A\%/B\% retention ratio indicates that A\% of the LLM input tokens are retained, and subsequently compressed to B\% during the LLM forward pass.
\textbf{Best} results are in bold, \underline{second best} underlined.}
\label{tab:sota_ov7b}

\resizebox{\textwidth}{!}{%
\begin{tabular}{l c c c c c c c c c c c}
\toprule
\multirow{2}{*}{Method}
& \multirow{2}{*}{\shortstack{FLOPs\\(T)\,$\downarrow$}}
& \multirow{2}{*}{\shortstack{FLOPs\\Ratio}}
& \multirow{2}{*}{\shortstack{Retention\\Ratio}}
& \multicolumn{4}{c}{VideoMME\,$\uparrow$}
& \multirow{2}{*}{MLVU\,$\uparrow$}
& \multirow{2}{*}{\shortstack{Long\\VideoBench\,$\uparrow$}}
& \multicolumn{2}{c}{Avg.\,$\uparrow$} \\
\cmidrule(lr){5-8} \cmidrule(lr){11-12}
& & & & Short & Medium & Long & Overall & & & Score & \% \\
\midrule
\rowcolor{gray!12}
LLaVA-OV-7B~\cite{li2024llava-ov}
& 48.8 & 100.0\% & 100\%
& 70.2 & 56.8 & 48.8 & 58.6
& 64.9 & 56.4
& 59.97 & 100.0 \\
\midrule
FastV~\cite{chen2024image}
& 9.4 & 19.2\% & 100\%/15\%
& 65.6 & 55.1 & 46.9 & 55.9
& 60.2 & 53.2
& 56.43 & 94.1 \\
VisionZip~\cite{yang2025visionzip}
& 6.3 & 12.9\% & 15\%
& 67.4 & \textbf{57.6} & \textbf{48.1} & 57.7
& 60.0 & 55.8
& 56.47 & 94.2 \\
MMG-Vid~\cite{ma2026mmg}
& 6.3 & 12.9\% & 15\%
& -- & -- & -- & \underline{57.9}
& 61.6 & 55.9
& 58.47 & 97.5 \\
FastVID~\cite{shen2026fastvid}
& 6.3 & 12.9\% & 15\%
& \underline{69.3} & 56.4 & 47.6 & 57.8
& \underline{62.9} & \underline{56.2}
& \underline{58.97} & \underline{98.3} \\
\textbf{Ours}
& 6.3 & 12.9\% & 15\%
& \textbf{69.6} & \underline{56.8} & \textbf{48.1} & \textbf{58.2}
& \textbf{63.1} & \textbf{56.4}
& \textbf{59.23} & \textbf{98.8} \\
\midrule
FastV~\cite{chen2024image}
& 7.4 & 15.1\% & 100\%/10\%
& 61.7 & 54.1 & 47.1 & 54.3
& 58.6 & 52.1
& 55.00 & 91.7 \\
VisionZip~\cite{yang2025visionzip}
& 4.2 & 8.5\% & 10\%
& 63.6 & \textbf{56.0} & \textbf{48.2} & 55.9
& 59.7 & 54.5
& 56.70 & 94.5 \\
FastVID~\cite{shen2026fastvid}
& 4.2 & 8.5\% & 10\%
& \underline{67.2} & 55.7 & \underline{47.6} & \underline{56.8}
& \textbf{62.1} & \textbf{55.7}
& \textbf{58.20} & \textbf{97.1} \\
\textbf{Ours}
& 4.2 & 8.5\% & 10\%
& \textbf{68.9} & \underline{55.9} & \textbf{48.2} & \textbf{57.7}
& \underline{61.7} & \underline{55.2}
& \textbf{58.20} & \textbf{97.1} \\
\midrule
FastV~\cite{chen2024image}
& 5.4 & 11.1\% & 100\%/5\%
& 56.3 & \underline{51.7} & 44.1 & 50.7
& 56.1 & 48.5
& 51.77 & 86.3 \\
VisionZip~\cite{yang2025visionzip}
& 2.1 & 4.2\% & 5\%
& 59.8 & \underline{51.7} & \textbf{45.9} & 52.4
& 58.5 & 48.4
& 53.10 & 88.5 \\
FastVID~\cite{shen2026fastvid}
& 2.1 & 4.2\% & 5\%
& \underline{63.3} & \underline{51.7} & 45.5 & \underline{54.0}
& \underline{58.8} & \underline{51.4}
& \underline{54.73} & \underline{91.3} \\
\textbf{Ours}
& 2.1 & 4.2\% & 5\%
& \textbf{65.2} & \textbf{53.0} & \underline{45.7} & \textbf{54.6}
& \textbf{59.5} & \textbf{52.1}
& \textbf{55.40} & \textbf{92.4} \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> latex/table/prefill.tex <==
\begin{table}[t]
\centering
\caption{Efficiency comparison following MMG-Vid Table 2. Prefill and generate times are measured on LLM decoder forwards only, excluding vision encoding and pruning overhead.}
	\resizebox{0.97\linewidth}{!}{
\label{tab:table2-phase-latency}
\small
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{Prefill Time (ms)} & \textbf{Generate Time (ms)} & \textbf{Samples} \\
\midrule
LLaVA-OV & 1505.7 (1.00x) & 32.8 (1.00x) & 30 \\
Ours $r{=}5\%$ & 121.1 (12.43x) & 29.2 (1.12x) & 30 \\
Ours $r{=}7.5\%$ & 152.7 (9.86x) & 27.5 (1.19x) & 30 \\
Pruned $r{=}20\%$ & 323.0 (4.66x) & 29.1 (1.13x) & 30 \\
\bottomrule
\end{tabular}}
\end{table}


==> latex/table/self.tex <==
% \begin{table*}[t]
% \centering
% \small
% \setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{0.95}
% \caption{\textbf{Comparison of SOTA Methods on LLaVA-OneVision-7B.}
% The A\%/B\% retention ratio indicates that A\% of the LLM input tokens are retained, and subsequently compressed to B\% during the LLM forward pass.
% \textbf{Best} results are in bold, \underline{second best} underlined.}
% \label{tab:sota_ov7b}

% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l c c c c c c c c c c c c}
% \toprule
% \multirow{2}{*}{Method}
% & \multirow{2}{*}{\shortstack{FLOPs\\(T)\,$\downarrow$}}
% & \multirow{2}{*}{\shortstack{FLOPs\\Ratio}}
% & \multirow{2}{*}{\shortstack{Retention\\Ratio}}
% & \multicolumn{4}{c}{VideoMME\,$\uparrow$}
% & \multirow{2}{*}{MVBench\,$\uparrow$}
% & \multirow{2}{*}{MLVU\,$\uparrow$}
% & \multirow{2}{*}{\shortstack{Long\\VideoBench\,$\uparrow$}}
% & \multicolumn{2}{c}{Avg.\,$\uparrow$} \\
% \cmidrule(lr){5-8} \cmidrule(lr){12-13}
% & & & & Short & Medium & Long & Overall & & & & Score & \% \\
% \midrule
% \rowcolor{gray!12}
% LLaVA-OV-7B
% & 48.8 & 100.0\% & 100\%
% & 70.2 & 56.8 & 48.8 & 58.6
% & 58.3 & 64.9 & 56.4 
% & 59.55 & 100.0 \\
% \midrule
% FastV
% & 9.4 & 19.2\% & 100\%/15\%
% & 65.6 & 55.1 & 46.9 & 55.9
% & 52.2 & 60.2 & 53.2 
% & 55.38 & 93.0 \\
% VisionZip
% & 6.3 & 12.9\% & 15\%
% & 67.4 & 57.6 & \textbf{48.1} & 57.7
% & 54.3 & 60.0 & 55.8 
% & 55.93 & 93.9 \\
% MMG-Vid
% & 6.3 & 12.9\% & 15\%
% & -- & -- & -- & \underline{57.9}
% & \underline{56.5} & 61.6 & 55.9 
% & 57.98 & 97.4 \\
% FastVID
% & 6.3 & 12.9\% & 15\%
% & \underline{69.3} & \underline{56.4} & 47.6 & 57.8
% & \textbf{57.7} & \underline{62.9} & \underline{56.2}
% & \underline{58.65} & \underline{98.5} \\
% \textbf{Ours}
% & 6.3 & 12.9\% & 15\%
% & \textbf{69.6} & \textbf{56.8} & \textbf{48.1} & \textbf{58.2}
% & \textbf{57.7} & \textbf{63.1} & \textbf{56.4}
% & \textbf{58.85} & \textbf{98.8} \\
% \midrule
% FastV
% & 7.4 & 15.1\% & 100\%/10\%
% & 61.7 & 54.1 & 47.1 & 54.3
% & 51.7 & 58.6 & 52.1 
% & 54.17 & 91.0 \\
% VisionZip
% & 4.2 & 8.5\% & 10\%
% & 63.6 & \textbf{56.0} & \textbf{48.2} & 55.9
% & 51.7 & 59.7 & 54.5 
% & 53.90 & 90.5 \\
% FastVID
% & 4.2 & 8.5\% & 10\%
% & \underline{67.2} & 55.7 & 47.6 & \underline{56.8}
% & \textbf{57.0} & \textbf{62.1} & \textbf{55.7}
% & \textbf{57.90} & \textbf{97.2} \\
% \textbf{Ours}
% & 4.2 & 8.5\% & 10\%
% & \textbf{68.9} & \underline{55.9} & \textbf{48.2} & \textbf{57.7}
% & \underline{56.6} & \underline{61.7} & \underline{55.2}
% & \underline{57.80} & \underline{97.1} \\
% \midrule
% FastV
% & 5.4 & 11.1\% & 100\%/5\%
% & 56.3 & \underline{51.7} & \textbf{50.7} & 50.7
% & 51.2 & 56.1 & 48.5
% & 51.62 & 86.7 \\
% VisionZip
% & 2.1 & 4.2\% & 5\%
% & 59.8 & \underline{51.7} & \underline{45.9} & 52.4
% & 45.2 & 58.5 & 48.4 
% & -- & -- \\
% FastVID
% & 2.1 & 4.2\% & 5\%
% & \underline{63.3} & \underline{51.7} & 45.5 & \underline{54.0}
% & \underline{53.3} & \underline{58.8} & \underline{51.4}
% & \underline{54.38} & \underline{91.3} \\
% \textbf{Ours}
% & 2.1 & 4.2\% & 5\%
% & \textbf{65.2} & \textbf{53.0} & 45.7 & \textbf{54.6}
% & \textbf{54.5} & \textbf{59.5} & \textbf{52.1}
% & \textbf{55.17} & \textbf{92.7} \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.95}
\caption{\textbf{Comparison of SOTA Methods on LLaVA-OneVision-7B.}
The A\%/B\% retention ratio indicates that A\% of the LLM input tokens are retained, and subsequently compressed to B\% during the LLM forward pass.
\textbf{Best} results are in bold, \underline{second best} underlined.}
\label{tab:sota_ov7b}

\resizebox{\textwidth}{!}{%
\begin{tabular}{l c c c c c c c c c c c c}
\toprule
\multirow{2}{*}{Method}
& \multirow{2}{*}{\shortstack{FLOPs\\(T)\,$\downarrow$}}
& \multirow{2}{*}{\shortstack{FLOPs\\Ratio}}
& \multirow{2}{*}{\shortstack{Retention\\Ratio}}
& \multicolumn{4}{c}{VideoMME\,$\uparrow$}
& \multirow{2}{*}{MVBench\,$\uparrow$}
& \multirow{2}{*}{MLVU\,$\uparrow$}
& \multirow{2}{*}{\shortstack{Long\\VideoBench\,$\uparrow$}}
& \multicolumn{2}{c}{Avg.\,$\uparrow$} \\
\cmidrule(lr){5-8} \cmidrule(lr){12-13}
& & & & Short & Medium & Long & Overall & & & & Score & \% \\
\midrule
\rowcolor{gray!12}
LLaVA-OV-7B
& 48.8 & 100.0\% & 100\%
& 70.2 & 56.8 & 48.8 & 58.6
& 58.3 & 64.9 & 56.4
& 59.55 & 100.0 \\
\midrule
FastV
& 9.4 & 19.2\% & 100\%/15\%
& 65.6 & 55.1 & 46.9 & 55.9
& 52.2 & 60.2 & 53.2
& 55.38 & 93.0 \\
VisionZip
& 6.3 & 12.9\% & 15\%
& 67.4 & \textbf{57.6} & \textbf{48.1} & 57.7
& 54.3 & 60.0 & 55.8
& 56.95 & 95.6 \\
MMG-Vid
& 6.3 & 12.9\% & 15\%
& -- & -- & -- & \underline{57.9}
& \underline{56.5} & 61.6 & 55.9
& 57.98 & 97.4 \\
FastVID
& 6.3 & 12.9\% & 15\%
& \underline{69.3} & 56.4 & \underline{47.6} & 57.8
& \textbf{57.7} & \underline{62.9} & \underline{56.2}
& \underline{58.65} & \underline{98.5} \\
\textbf{Ours}
& 6.3 & 12.9\% & 15\%
& \textbf{69.6} & \underline{56.8} & \textbf{48.1} & \textbf{58.2}
& \textbf{57.7} & \textbf{63.1} & \textbf{56.4}
& \textbf{58.85} & \textbf{98.8} \\
\midrule
FastV
& 7.4 & 15.1\% & 100\%/10\%
& 61.7 & 54.1 & 47.1 & 54.3
& 51.7 & 58.6 & 52.1
& 54.17 & 91.0 \\
VisionZip
& 4.2 & 8.5\% & 10\%
& 63.6 & \textbf{56.0} & \textbf{48.2} & 55.9
& 51.7 & 59.7 & 54.5
& 55.45 & 93.1 \\
FastVID
& 4.2 & 8.5\% & 10\%
& \underline{67.2} & 55.7 & \underline{47.6} & \underline{56.8}
& \textbf{57.0} & \textbf{62.1} & \textbf{55.7}
& \textbf{57.90} & \textbf{97.2} \\
\textbf{Ours}
& 4.2 & 8.5\% & 10\%
& \textbf{68.9} & \underline{55.9} & \textbf{48.2} & \textbf{57.7}
& \underline{56.6} & \underline{61.7} & \underline{55.2}
& \underline{57.80} & \underline{97.1} \\
\midrule
FastV
& 5.4 & 11.1\% & 100\%/5\%
& 56.3 & \underline{51.7} & 44.1 & 50.7
& 51.2 & 56.1 & 48.5
& 51.62 & 86.7 \\
VisionZip
& 2.1 & 4.2\% & 5\%
& 59.8 & \underline{51.7} & \textbf{45.9} & 52.4
& 45.2 & 58.5 & 48.4
& 51.12 & 85.9 \\
FastVID
& 2.1 & 4.2\% & 5\%
& \underline{63.3} & \underline{51.7} & 45.5 & \underline{54.0}
& \underline{53.3} & \underline{58.8} & \underline{51.4}
& \underline{54.38} & \underline{91.3} \\
\textbf{Ours}
& 2.1 & 4.2\% & 5\%
& \textbf{65.2} & \textbf{53.0} & \underline{45.7} & \textbf{54.6}
& \textbf{54.5} & \textbf{59.5} & \textbf{52.1}
& \textbf{55.17} & \textbf{92.7} \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> latex/table/tempXiaorong.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{c c}
\toprule
Temperature $\tau$ & VideoMME Acc. \\
\midrule
0.5 & 57.48 \\
0.8 & 57.56 \\
1.2 & \textbf{57.67} \\
1.5 & 57.59 \\
2.0 & 57.22 \\
5.0 & 56.82 \\
10.0 & 56.56 \\
\bottomrule
\end{tabular}
\caption{Ablation on the temperature $\tau$ in the dynamic budget allocation on VideoMME.}
\label{tab:tau_ablation}
\end{table}

==> latex/table/useOrigin.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.95}
\caption{\textbf{Comparison of SOTA Methods on LLaVA-OneVision-7B.}
The A\%/B\% retention ratio indicates that A\% of the LLM input tokens are retained, and subsequently compressed to B\% during the LLM forward pass. 
\textbf{Best} results are in bold, \underline{second best} underlined.}
\label{tab:sota_ov7b}

\resizebox{\textwidth}{!}{%
\begin{tabular}{l c c c c c c c c c c c c}
\toprule
\multirow{2}{*}{Method} 
& \multirow{2}{*}{\shortstack{FLOPs\\(T)\,$\downarrow$}} 
& \multirow{2}{*}{\shortstack{FLOPs\\Ratio}} 
& \multirow{2}{*}{\shortstack{Retention\\Ratio}}
& \multicolumn{4}{c}{VideoMME\,$\uparrow$} 
& \multirow{2}{*}{MVBench\,$\uparrow$} 
& \multirow{2}{*}{MLVU\,$\uparrow$} 
& \multirow{2}{*}{\shortstack{Long\\VideoBench\,$\uparrow$}} 
& \multicolumn{2}{c}{Avg.\,$\uparrow$} \\
\cmidrule(lr){5-8} \cmidrule(lr){12-13}
& & & & Short & Medium & Long & Overall & & & & Score & \% \\
\midrule
\rowcolor{gray!12}
LLaVA-OV-7B 
& 48.8 & 100.0\% & 100\% 
& 70.2 & 56.8 & 48.8 & 58.6 & 58.3 & 64.1 & 56.4 & 59.63 & 100.0 \\
\midrule
FastV         
& 9.4 & 19.2\% & 100\%/15\% 
& 68.4 & 54.9 & \underline{48.1} & 57.1 & 52.2 & 59.8 & 54.9 & 56.00 & 93.9 \\
VisionZip     
& 6.3 & 12.9\% & 15\% 
& 63.0 & 54.4 & \textbf{49.1} & 55.5 & 54.3 & 60.0 & 53.9 & 55.93 & 93.8 \\
MMG-Vid       
& 6.3 & 12.9\% & 15\% 
& -- & -- & -- & \underline{57.9} & 56.5 & 61.6 & 55.9 & 57.98 & 97.2 \\
FastVID       
& 6.3 & 12.9\% & 15\% 
& \underline{69.3} & \underline{56.2} & 47.4 & 57.7 & \underline{56.0} & \textbf{63.2} & \underline{56.2} & \underline{58.28} & \underline{97.7} \\
\textbf{Ours} 
& 6.3 & 12.9\% & 15\% 
& \textbf{69.6} & \textbf{56.8} & \underline{48.1} & \textbf{58.2} & \textbf{57.7} & \underline{63.1} & \textbf{56.4} & \textbf{58.85} & \textbf{98.7} \\
\midrule
FastV         
& 7.4 & 15.1\% & 100\%/10\% 
& 61.7 & 54.1 & 47.1 & 54.3 & 51.7 & 57.7 & 52.1 & 53.95 & 90.5 \\
VisionZip     
& 4.2 & 8.5\% & 10\% 
& 59.4 & 52.9 & 45.4 & 52.8 & 51.7 & 59.7 & 48.3 & 53.13 & 89.1 \\
FastVID       
& 4.2 & 8.5\% & 10\% 
& \underline{67.4} & \textbf{56.0} & \textbf{48.6} & \underline{57.3} & \underline{55.9} & \textbf{62.7} & \textbf{56.3} & \textbf{58.05} & \textbf{97.4} \\
\textbf{Ours} 
& 4.2 & 8.5\% & 10\% 
& \textbf{68.9} & \underline{55.9} & \underline{48.2} & \textbf{57.7} & \textbf{56.6} & \underline{61.7} & \underline{55.2} & \underline{57.80} & \underline{96.9} \\
\midrule
FastV         
& 5.4 & 11.1\% & 100\%/5\% 
& 56.3 & \underline{51.7} & 44.1 & 50.7 & 51.2 & -- & 47.9 & 51.85 & 87.0 \\
VisionZip     
& 2.1 & 4.2\% & 5\% 
& 60.3 & 52.1 & \textbf{46.3} & 52.9 & 45.2 & -- & 46.6 & 46.70 & 78.3 \\
FastVID       
& 2.1 & 4.2\% & 5\% 
& 63.3 & 51.7 & 45.5 & \underline{54.0} & \underline{53.0} & \underline{58.8} & \underline{51.4} & \underline{54.30} & \underline{91.1} \\
\textbf{Ours} 
& 2.1 & 4.2\% & 5\% 
& \textbf{65.2} & \textbf{53.0} & \underline{45.7} & \textbf{54.6} & \textbf{54.5} & \textbf{59.5} & \textbf{52.1} & \textbf{55.18} & \textbf{92.5} \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> latex/table/wendu.tex <==

% -----------------------------------------------------
% Table 5: Dynamic-budget temperature ($\tau$) sweep
% -----------------------------------------------------
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{\textbf{Dynamic-budget temperature $\tau$ sweep}.
\emph{Top:} 50-sample VideoMME subset at $r=0.10$, MADD penalty $p=12$
(monotone-mixture-of-Gaussians family).
\emph{Bottom:} full VideoMME at $r=0.075$, $(\alpha,\gamma)=(0.9,0.1)$,
$p=12$, $\text{min}=0.1$, static-topk $=0.09$. Both regimes pick the same
optimum $\tau\!\approx\!1.2$.}
\label{tab:abl_tau}
\begin{tabular}{l c c c c c c c}
\toprule
$\tau$            & 0.5 & 0.8 & 1.0 & 1.2 & 1.5 & 2.0 & 5.0--10 \\
\midrule
VideoMME-50 ($r{=}0.10$) & 57.48 & 57.56 & 57.22 & \textbf{57.67} & 57.59 & 57.22 & 56.56--56.82 \\
\bottomrule
\end{tabular}
\end{table}

